Accuracy of Gaussian approximation in nonparametric Bernstein -- von Mises Theorem

The prominent Bernstein -- von Mises (BvM) result claims that the posterior distribution after centering by the efficient estimator and standardizing by the square root of the total Fisher information is nearly standard normal. In particular, the prior completely washes out from the asymptotic posterior distribution. This fact is fundamental and justifies the Bayes approach from the frequentist viewpoint. In the nonparametric setup the situation changes dramatically and the impact of prior becomes essential even for the contraction of the posterior; see [vdV2008], [Bo2011], [CaNi2013,CaNi2014] for different models like Gaussian regression or i.i.d. model in different weak topologies. This paper offers another non-asymptotic approach to studying the behavior of the posterior for a special but rather popular and useful class of statistical models and for Gaussian priors. First we derive tight finite sample bounds on posterior contraction in terms of the so called effective dimension of the parameter space. Our main results describe the accuracy of Gaussian approximation of the posterior. In particular, we show that restricting to the class of all centrally symmetric credible sets around pMLE allows to get Gaussian approximation up to order (n^{-1}). We also show that the posterior distribution mimics well the distribution of the penalized maximum likelihood estimator (pMLE) and reduce the question of reliability of credible sets to consistency of the pMLE-based confidence sets. The obtained results are specified for nonparametric log-density estimation and generalized regression.

==> A_gauss_int.tex <==
% !TEX root = ../pa_np_bvm.tex

\section{Gaussian integrals}
\label{SGaussintegr}
Let \( \TAU \) be a linear mapping in \(\R^{\dimp}\) with \(\| \TAU \|_{\oper} \leq 1\).
Given positive \(\rups\) and \(\CONSTru\), consider the following ratio of two integrals
\begin{EQA}[c]
\frac{\int_{\| \TAU \uv \| > \rups}
\exp\bigl(
  - \CONSTru \| \TAU \uv \| + \frac{1}{2} \CONSTru \rups^{2}
  + \frac{1}{2} \| \TAU \uv \|^{2} 
  - \frac{1}{2} \| \uv \|^{2} 
\bigr) d\uv}
{\int_{\| \TAU \uv \| \leq \rups}
\exp\bigl( - \frac{1}{2}\| \uv \|^{2} \bigr) d\uv} \, .
\label{AAuvrupsc}
\end{EQA}
%
Obviously, one can rewrite this value as ratio of two expectations
\begin{EQA}[c]
	\frac{\E \Bigl\{ \exp\bigl(	- \CONSTru \rups \| \TAU \gaussv \| 
			+ \frac{1}{2} \CONSTru \rups^{2}
  			+ \frac{1}{2} \| \TAU \gaussv \|^{2} \bigr) 
			\Ind\bigl( \| \TAU \gaussv \| > \rups \bigr) \Bigr\}}
		 {\P\bigl( \| \TAU \gaussv \| \leq \rups \bigr) } \, .
\label{EindAAgelerr}
\end{EQA}
%
Note that without the linear term \(- \CONSTru \| \TAU \gaussv \|\) in the exponent, 
the expectation in the numerator can be infinite. 
We aim at describing \(\rups\) and \(\CONSTru\)-values which ensure that 
the probability in denominator is close to one while the expectation in the numerator is small.

\begin{lemma}
\label{TGaussintext}
Let \(\TAU\) be a linear operator in \(\R^{\dimp}\)-matrix with 
\(\| \TAU \|_{\oper} \leq 1\).
Define \(\dimAA = \tr(\TAU^{\T} \TAU)\).
%     and \(\vA = (\dimA + \xx)^{1/2} + (\dimA + \xx)^{-1/2}\).
For any \(\CONSTru, \rups\) with 
\(1/2 < \CONSTru \leq 1\) and 
\(\CONSTru \rups = 2 \sqrt{\dimAA} + \sqrt{\xx} \) for \( \xx > 0 \) 
\begin{EQA}
% && \nquad
  \E \Bigl\{ \exp\Bigl(
    		- \CONSTru \rups \| \TAU \gaussv \| + \frac{\CONSTru \rups^{2}}{2}
    		+ \frac{1}{2} \| \TAU \gaussv \|^{2} 
  	\Bigr) \Ind\bigl( \| \TAU \gaussv \| > \rups \bigr) \Bigr\}
% \\
  	& \leq &
% \exp\Bigl( - \frac{a \rups \vA + \vA^{2}}{2} \Bigr) ,
	\CONST \ex^{ - (\dimAA + \xx)/2}
\label{EexCruAg12Ag2}
\end{EQA}
and 
\begin{EQA}
  \P\bigl( \| \TAU \gaussv \| \leq \rups \bigr)
  & \geq &
  1 - \exp \Bigl\{ - \frac{1}{2} (\rups - \sqrt{\dimAA})^{2} \Bigr\}
  \geq 
  1 - \ex^{- \dimAA - \xx}.
\label{EeAg12Ag2}
\end{EQA}
\end{lemma}

\begin{remark}
The result applies even if the full dimension \(\dimp\) is infinite and \(\gaussv\) is a Gaussian element in a Hilbert space, provided that \(\dimAA = \tr(\TAU^{\T} \TAU)\) is finite, that is, \(\TAU^{\T} \TAU\) is a trace operator.
\end{remark}

\begin{proof}
Define
\begin{EQA}
	\PAAr(\rr)
	& \eqdef &
	\P\bigl( \| \TAU \gaussv \| \geq \rr \bigr),
	\\
	f(\rr)
	& \eqdef &
	\exp \Bigl( 
		- \CONSTru \rups \rr + \frac{\CONSTru \rups^{2}}{2} + \frac{\rr^{2}}{2} 
	\Bigr)
\label{PhirPAgrfrC0}
\end{EQA}
Then
\begin{EQA}
	&& \nquad
	\E \Bigl\{ \exp\Bigl(
        - \CONSTru \rups \| \TAU \gaussv \| + \frac{\CONSTru \rups^{2}}{2}
        + \frac{1}{2} \| \TAU \gaussv \|^{2} 
      \Bigr) \Ind\bigl( \| \TAU \gaussv \| > \rups \bigr) \Bigr\}
    \\
    &=&
    - \int_{\rups}^{\infty} f(\rr) d\PAAr(\rr)
    =
    - f(\rups) \PAAr(\rups)
    + \int_{\rups}^{\infty} f'(\rr) \PAAr(\rr) \, d\rr \, .
\label{irifpPhrdrf}
\end{EQA}
Now we use that
\( \PAAr\bigl( \sqrt{\dimAA} + \sqrt{2\xx} \bigr) \leq \ex^{-\xx} \)
for any \( \xx > 0 \).
This can be rewritten as
\begin{EQA}
	\PAAr(\rr)
	& \leq &
	\exp \Bigl\{ - \frac{1}{2} \bigl( \rr - \sqrt{\dimAA} \bigr)^{2} \Bigr\}
\label{Pr12rsA2mr}
\end{EQA}
for \( \rr > \sqrt{\dimAA} \).
Now we use that \( f'(\rr) = (\rr - \CONSTru \rups) f(\rr) \) and 
\begin{EQA}
	\int_{\rups}^{\infty} f'(\rr) \PAAr(\rr) \, d\rr
	&=&
	\int_{\rups}^{\infty} (\rr - \CONSTru \rups) f(\rr) \PAAr(\rr) \, d\rr
	\\
	& \leq &
	\int_{\rups}^{\infty} (\rr - \CONSTru \rups) 
		\exp\Bigl\{ - \frac{1}{2} \bigl( \rr - \sqrt{\dimAA} \bigr)^{2} 
			- \CONSTru \rups \rr + \frac{\CONSTru \rups^{2}}{2} + \frac{\rr^{2}}{2}
		\Bigr\} \, d\rr
	\\
	&=&
	\int_{\rups}^{\infty} (\rr - \CONSTru \rups) 
		\exp\Bigl\{ 
			- \bigl( \CONSTru \rups - \sqrt{\dimAA} \bigr) \rr 
			+ \frac{\CONSTru \rups^{2}}{2} - \frac{\dimAA}{2} 
		\Bigr\} \, d\rr
	\\
	&=&
	\int_{0}^{\infty} (x + \rups - \CONSTru \rups) 
		\exp\Bigl\{ 
			- \bigl( \CONSTru \rups - \sqrt{\dimAA} \bigr) (x + \rups) 
			+ \frac{\CONSTru \rups^{2}}{2} - \frac{\dimAA}{2} 
		\Bigr\} \, dx .
\label{i0iex0ixexd}
\end{EQA}
The use of \( \int_{0}^{\infty} \ex^{-x} dx = \int_{0}^{\infty} x \ex^{-x} dx = 1 \)
yields
\begin{EQA}
	\int_{\rups}^{\infty} f'(\rr) \PAAr(\rr) \, d\rr
	& \leq &
	\left( 
		\frac{\rups - \CONSTru \rups}{\CONSTru \rups - \sqrt{\dimAA}} 
		+ \frac{1}{(\CONSTru \rups - \sqrt{\dimAA})^{2}} 
	\right)
	\exp\Bigl\{ \rups \sqrt{\dimAA} 
			- \frac{\CONSTru \rups^{2}}{2} - \frac{\dimAA}{2} \Bigr\} .
\label{irifprPr222}
\end{EQA}
It remains to check that for \( \CONSTru \in (1/2,1) \)
and \( \CONSTru \rups = 2\sqrt{\dimAA} + \sqrt{\xx} \)
\begin{EQA}
	- \rups \sqrt{\dimAA} 
			+ \frac{\CONSTru \rups^{2}}{2} + \frac{\dimAA}{2}
	& \geq &
	\frac{\xx + \dimAA}{2} \, .
\label{xp2r0sQfr2}
\end{EQA}
\end{proof}

%  Now we slightly extend the result.
%%   and consider the case of a shifted vector \(\gaussv\).
%
%  \begin{lemma}
%  \label{TGaussintextxiv}
%    Let \(\biasv \in \R^{\dimp}\), \(1/2 < \CONSTru \leq 1\), and 
%    \begin{EQA}
%      \CONSTru \rups 
%      & \geq &
%      2 \bigl( \sqrt{\dimAA} + \| \TAU \biasv \| \bigr) .
%    \label{rupsGintbb}
%    \end{EQA}
%    %
%    Then 
%    \begin{EQA}
%      && \nquad
%      \E \Bigl\{ \exp\bigl(
%        - \CONSTru \rups \| \TAU \gaussv \| + \frac{1}{2} \CONSTru \rups^{2} 
%        + \frac{1}{2} \| \TAU \gaussv  \|^{2} + \biasv^{\T} \gaussv
%      \bigr) \Ind\bigl( \| \TAU \gaussv \| > \rups \bigr) \Bigr\}
%      \\
%      & \leq &
%      \CONST \exp\Bigl( 
%      - \frac{\dimAA + \xx - \| \bv \|^{2}}{2} 
%%      + \frac{\| \bv \|^{2}}{2} 
%    \Bigr).
%    \label{EeAg12Ag2xivb}
%    \end{EQA}
%  \end{lemma}
%\begin{proof}
%We follow the line of the proof of Lemma~\ref{TGaussintext}.
%Define
%\begin{EQA}
%	\PAArb(\rr)
%	& \eqdef &
%	\E \exp\bigl( \bv^{\T} \gaussv \bigr) \Ind\bigl( \| \TAU \gaussv \| \geq \rr \bigr),
%	\\
%	f(\rr)
%	& \eqdef &
%	\exp \Bigl( 
%		- \CONSTru \rups \rr + \frac{\CONSTru \rups^{2}}{2} + \frac{\rr^{2}}{2} 
%	\Bigr)
%\label{PhirEbvgAgrfrC0}
%\end{EQA}
%Then
%\begin{EQA}
%	&& \nquad
%	\E \Bigl\{ \exp\Bigl(
%        - \CONSTru \rups \| \TAU \gaussv \| + \frac{\CONSTru \rups^{2}}{2}
%        + \frac{1}{2} \| \TAU \gaussv \|^{2} + \bv^{\T} \gaussv 
%      \Bigr) \Ind\bigl( \| \TAU \gaussv \| > \rups \bigr) \Bigr\}
%    \\
%    &=&
%    - \int_{\rups}^{\infty} f(\rr) d\PAArb(\rr)
%    =
%    - f(\rups) \PAArb(\rups)
%    + \int_{\rups}^{\infty} f'(\rr) \PAArb(\rr) \, d\rr \, .
%\label{irifpbvPhrdrf}
%\end{EQA}
%For a fixed \( \rr > \sqrt{\dimAA} + \| \TAU \bv \| \), by \eqref{Pr12rsA2mr}
%\begin{EQA}
%	\PAArb(\rr)
%	& = &
%	\frac{1}{(2\pi)^{\dimp/2}} \int \exp\Bigl( \bv^{\T} \gaussv - \frac{\| \gaussv \|^{2}}{2} \Bigr)
%	 	\Ind\bigl( \| \TAU \gaussv \| > \rr \bigr) d \gaussv
%	\\
%	&=&
%	\frac{\ex^{\| \bv \|^{2}/2}}{(2\pi)^{\dimp/2}} 
%	\int \exp\Bigl( - \frac{\| \gaussv - \bv \|^{2}}{2} \Bigr)
%	 	\Ind\bigl( \| \TAU \gaussv \| > \rr \bigr) d \gaussv
%	\\
%	&=&
%	\ex^{\| \bv \|^{2}/2} \P\bigl( \| \TAU (\gaussv + \bv) \| > \rr  \bigr)
%	\\
%	& \leq &
%	\ex^{\| \bv \|^{2}/2} \P\bigl( \| \TAU \gaussv \| > \rr - \| \TAU \bv \| \bigr)
%	\\
%	&=&
%	\ex^{\| \bv \|^{2}/2} \PAAr(\rr - \| \TAU \bv \|) 
%	\leq 
%%	\ex^{\| \bv \|^{2}/2} 
%	\exp \Bigl\{ - \frac{1}{2} \bigl( \rr - \sqrt{\dimAA} - \| \TAU \bv \| \bigr)^{2} 
%		+ \frac{\| \bv \|^{2}}{2}
%	\Bigr\} .
%\label{eb22PAgrAb}
%\end{EQA}
%Now we can continue as in the proof of Lemma~\ref{TGaussintext} with 
%\( \sqrt{\dimAA} \) replaced by \( \sqrt{\dimAA} + \| \TAU \bv \| \) yielding
%\begin{EQA}
%	&& \nquad
%	\E \Bigl\{ \exp\bigl(
%        - \CONSTru \rups \| \TAU \gaussv \| + \frac{1}{2} \CONSTru \rups^{2} 
%        + \frac{1}{2} \| \TAU \gaussv  \|^{2} + \biasv^{\T} \gaussv
%    \bigr) \Ind\bigl( \| \TAU \gaussv \| > \rups \bigr) \Bigr\}
%    \\
%    & \leq &
%    \CONST \exp\Bigl( 
%      - \frac{\bigl( \sqrt{\dimAA} + \| \TAU \bv \| \bigr)^{2} + \xx }{2} 
%      + \frac{\| \bv \|^{2}}{2} 
%    \Bigr) 
%    \leq 
%    \CONST \exp\Bigl( 
%      - \frac{\dimAA + \xx }{2} 
%      + \frac{\| \bv \|^{2}}{2} 
%    \Bigr) 
%\label{b22CspA212}
%\end{EQA}
%as required.
%\end{proof}
%

Now we consider Gaussian integrals with an additional quadratic multiplier.
\begin{lemma}
\label{TGaussintextquad}
Let \( \TAU \) be a linear operator in \(\R^{\dimp}\) with \(\| \TAU \|_{\oper} \leq 1\).
Let \(\lambdav \in \R^{\infty}\) be a unit norm vector: \(\|\lambdav\| = 1\).
Define \(\dimAA = \tr(\TAU^{\T} \TAU)\).
For any positive \(\CONSTru, \rups\) with 
\(1/2 < \CONSTru \leq 1\) and 
\(\CONSTru \rups > 2 \sqrt{\dimAA+1} + \sqrt{\yy}\) 
\begin{EQA}
%  	\nquad
%  	&&
  	\E \Bigl\{|\lambdav^{\T} \gaussv|^2 \exp\Bigl(
    - \CONSTru \rups \| \TAU \gaussv \| + \frac{\CONSTru \rups^{2}}{2}
    + \frac{1}{2} \| \TAU \gaussv \|^{2} 
  	\Bigr) \Ind\bigl( \| \TAU \gaussv \| > \rups \bigr) \Bigr\} 
   	& \leq &
  	\CONST \ex^{ - (\dimAA + \yy)/2}.
\end{EQA}
\end{lemma}
  
  \begin{proof}
Define \( \AAla \) by \( \AAla^{\T} \AAla = \TAU^{\T} \TAU + \lambdav \lambdav^{\T} \).
Obviously \( \| \AAla \gaussv \| \geq \| \TAU \gaussv \| \),
\( |\lambdav^{\T} \gaussv| \leq \| \TAU \gaussv \| \).
Further, \( \rr^{2}/2 - \CONSTru \rups \rr \) grows in \( \rr \geq \rups \)
in view of \( \CONSTru \leq 1 \).
Therefore,
\begin{EQA}
	&& \nquad
	|\lambdav^{\T} \gaussv|^{2} \exp\Bigl(
        - \CONSTru \rups \| \TAU \gaussv \| + \frac{\CONSTru \rups^{2}}{2}
        + \frac{1}{2} \| \TAU \gaussv \|^{2} 
      \Bigr) \Ind\bigl( \| \TAU \gaussv \| > \rups \bigr)  
    \\
    & \leq &
    \| \AAla \gaussv \|^{2} \exp\Bigl(
        - \CONSTru \rups \| \AAla \gaussv \| + \frac{\CONSTru \rups^{2}}{2}
        + \frac{1}{2} \| \AAla \gaussv \|^{2} 
      \Bigr) \Ind\bigl( \| \AAla \gaussv \| > \rups \bigr)   
\label{•}
\end{EQA}
%
Now we can follow the line of the proof of Lemma~\ref{TGaussintext}.
Consider
\begin{EQA}
	\PAArg(\rr)
	& = &
	\P\bigl( \| \AAla \gaussv \| \geq \rr \bigr)
	\leq 
	\exp\bigl\{ - \frac{1}{2} (\rr - \sqrt{\dimAla}) \bigr\},
	\\
	f(\rr)
	& \eqdef &
	\rr^{2} \exp \Bigl( 
		- \CONSTru \rups \rr + \frac{\CONSTru \rups^{2}}{2} + \frac{\rr^{2}}{2} 
	\Bigr) 
\label{PhirElagAgrfrC0r2}
\end{EQA}
with \( \dimAla \eqdef \tr \AAla^{\T} \AAla = \dimA + 1 \).
Then
\begin{EQA}
	&& \nquad
	\E \Bigl\{ \bigl( \lambdav^{\T} \gaussv \bigr)^{2} \exp\Bigl(
        - \CONSTru \rups \| \TAU \gaussv \| + \frac{\CONSTru \rups^{2}}{2}
        + \frac{1}{2} \| \TAU \gaussv \|^{2}  
      \Bigr) \Ind\bigl( \| \TAU \gaussv \| > \rups \bigr) \Bigr\}
    \\
    & \leq &
    - \int_{\rups}^{\infty} f(\rr) d\PAArg(\rr)
    =
    - f(\rups) \PAArg(\rups)
    + \int_{\rups}^{\infty} f'(\rr) \PAArg(\rr) \, d\rr \, .
\label{irifplaPhrdrf}
\end{EQA}
Now we can continue as in the proof of Lemma~\ref{TGaussintext}.
\end{proof}

%\begin{lemma}
%\label{TGaussintextquadbias}
%Let \(\TAU\) be a linear operator in \(\R^{\infty}\) with \(\| \TAU \|_{\oper} \leq 1\).
%Let \(\biasv \in \R^{\infty}\) and also \(\lambdav \in \R^{\infty}\) be a unit norm vector: \(\|\lambdav\| = 1\).
%Define \(\dimAA = \tr(\TAU^{\T} \TAU)\) and \(\vA = (\dimAA + 1 + \xx)^{1/2} + (\dimAA + 1 + \xx)^{-1/2}\).
%For any positive \(\CONSTru, \rups\) with \(1/2 < \CONSTru \leq 1\) and \(\CONSTru \rups > 4 \vA + 2\|\AA\biasv\|\) it holds
%\begin{EQA}[c]
%  \nquad
%  \E \Bigl\{|\lambdav^{\T} \gaussv|^2 \exp\Bigl(
%    - \CONSTru \rups \| \TAU (\gaussv - \biasv) \| + \frac{\CONSTru \rups^{2}}{2}
%    + \frac{1}{2} \| \TAU (\gaussv- \biasv)\|^{2} 
%  \Bigr) \Ind\bigl( \| \TAU (\gaussv-\biasv) \| > \rups \bigr) \Bigr\} 
%   \leq 
%  \ex^{-2\xx}.
%\end{EQA}
%\end{lemma}
%
%\begin{proof}
%Proof is similar to the proof of Lemma~\ref{TGaussintextquad}. 
%%    Theorem~\ref{TGaussintextquadbias} is proved.
%\end{proof}


==> A_proof_lin.tex <==
% !TEX root = ../gpp_linear.tex

\section{Proofs of the main results}
This section collects the proofs of the main theorems.


\subsection{Proof of Theorem~\ref{Thyperpost2}}

The first fact provides a simple and useful representation of the 
hyper-posterior.

\begin{proposition}
\label{Lhyperbpr}
With \( \tilde{\thetav}_{\hyper} = \tilde{\thetav}_{\GP_{\hyper}} \) and 
\( \DP_{\hyper}^{2} = \DP_{\GP_{\hyper}}^{2} \) from \eqref{IFGPdefBvMig}, 
\begin{EQA}
	\hyper \cond \Yv
	& \sim &
	\frac{\priorh_{\hyper} \exp\bigl\{ L_{\hyper}(\tilde{\thetav}_{\hyper}) 
			- \penm_{\hyper}/2 \bigr\}}
		 {\sum_{\hyper \in \MM} \priorh_{\hyper} \exp\bigl\{ L_{\hyper}(\tilde{\thetav}_{\hyper})
		 	- \penm_{\hyper}/2 \bigr\}} \, ,
\label{hcYcGapGaLGa1}
\end{EQA}
where 
\begin{EQA}
	\penm_{\hyper}
	& \eqdef &
	- \log\frac{\det \GP_{\hyper}^{2} }{\det \DP_{\hyper}^{2}} \, .
\label{cGaeldGadDGa}
\end{EQA}
\end{proposition}

\begin{proof}
Let us fix any \( \hyper \in \MM \).
Remind that with 
\( \DP_{\hyper}^{2} = \sigma^{-2} \Psi \Psi^{\T} + \GP_{\hyper}^{2} \), 
it holds for any \( \thetavd \) by quadraticity of \( L_{\hyper}(\thetav) \) in 
\( \thetav \) that
\begin{EQA}
	L_{\hyper}(\tilde{\thetav}_{\hyper}) - L_{\hyper}(\thetav)
	&=&
	\sup_{\thetavc} L_{\hyper}(\thetavc) - L(\thetav)
	=
	\frac{\bigl\| \DP_{\hyper} \bigl( \tilde{\thetav}_{\hyper} - \thetav \bigr) \bigr\|^{2}}{2} .
\label{LGttGLGtdsLDG2}
\end{EQA}
Now we derive
\begin{EQA}
	\int \exp\bigl\{ L_{\hyper}(\thetav) \bigr\} d\thetav
	&=&
	\exp\bigl\{ L_{\hyper}(\tilde{\thetav}_{\hyper}) \bigr\}
	\int \exp\bigl\{ L_{\hyper}(\thetav) - L_{\hyper}(\tilde{\thetav}_{\hyper}) \bigr\} d\thetav
	\\
	&=&
	\exp\bigl\{ L_{\hyper}(\tilde{\thetav}_{\hyper}) \bigr\}
	\int \exp\bigl\{ - \| \DP_{\hyper} (\tilde{\thetav}_{\hyper} - \thetav) \|^{2}/2 \bigr\} d\thetav
	\\
	& \propto &
	\frac{1}{\det \DP_{\hyper}} \exp\bigl\{ L_{\hyper}(\tilde{\thetav}_{\hyper}) \bigr\} 
\label{1dDGaeLGttGa}
\end{EQA}
and the assertion follows from \eqref{hYpGaieLGlddt}.
\end{proof}



Let us fix some \( \hyper \in \MM \) and denote \( \GP = \GP_{\hyper} \).
We begin by the following decomposition which
provides a more detailed description of each term 
\( L_{\GP}(\tilde{\thetav}_{\GP}) - \penm_{\GP}/2 \). 

\begin{proposition}
\label{Phyperprdec}
Let \( \fvs \eqdef \E \Yv \) and \( \epsv = \Yv - \E \Yv \) with \( \Var(\epsv) = \sigma^{2} \Id_{n} \). 
For each \( \hyper \in \MM \) and \( \GP = \GP_{\hyper} \)
\begin{EQA}
	L_{\GP}(\tilde{\thetav}_{\GP}) - \frac{\penm_{\GP}}{2}
	&=&
	- \frac{1}{2} \bigl( \varA_{\GP}^{2} + \bias_{\GP}^{2} \bigr) + \frac{\zeta_{\GP}}{2} + \CONST ,
\label{2efPf22x2Ex2}
\end{EQA}
where \( \CONST \) does not depend on \( \fvs \) or \( \GP \),  
\begin{EQA}
	\varA_{\GP}^{2}
	& \eqdef &
	\penm_{\GP} - \dimA_{\GP} 
	=
	- \log\frac{\det \GP^{2} }{\det \DP^{2}_{\GP}} 
	- \tr\bigl( \DP_{\GP}^{-1} \DPc^{2} \DP_{\GP}^{-1} \bigr)
	\geq 
	\frac{1}{2} \tr\bigl( \DP_{\GP}^{-1} \DPc^{2} \DP_{\GP}^{-1} \bigr)^{2} \, ,
	\\
\label{sm1m2Dm1LGts}
	\bias_{\GP}^{2}
	&=&
	\bias_{\GP}^{2}(\fvs)
	\eqdef 
%	\sigma^{-2} \| \fvs - \Pi_{\GP} \fvs \|^{2} + \bigl\| \GP \thetavsGP \bigr\|^{2} 
%	=
	\sigma^{-2} \bigl\langle \fvs, (\Id - \Pi_{\GP}) \fvs \bigr\rangle
%	\sigma^{-2} \| \fvs - \Pi_{\GP} \fvs \|^{2} 
%	+ \bigl\| \GP \bigl( \Psi \Psi^{\T} + \sigma^{2} \GP^{2} \bigr)^{-1} \Psi \fvs \bigr\|^{2}
\end{EQA} 
for \( \Pi_{\GP} = \Psi^{\T} \bigl( \Psi \Psi^{\T} + \sigma^{2} \GP^{2} \bigr)^{-1} \Psi \).
The stochastic term \( \zeta_{\GP} = \zeta_{\GP}(\epsv) \) in \eqref{2efPf22x2Ex2} is 
\begin{EQA}
	\zeta_{\GP}
	& \eqdef & 
	\bigl\| \xiv_{\GP} \bigr\|^{2} - \E \bigl\| \xiv_{\GP} \bigr\|^{2}
	+ \frac{2}{\sigma^{2}} \bigl\langle \epsv, \fvs - \Pi_{\GP} \fvs \bigr\rangle 
\label{12s2Ee22lrf}
\end{EQA}
for 
\begin{EQA}
	\xiv_{\GP} 
	& \eqdef & 
	\sigma^{-2} \DP_{\GP}^{-1} \Psi \epsv
	=
	\sigma^{-1} \bigl( \Psi \Psi^{\T} + \sigma^{2} \GP^{2} \bigr)^{-1/2} \Psi \epsv .
\label{xiGsm2DGm1Pev}
\end{EQA}
\end{proposition}




\begin{proof}
Given \( \GP^{2} > 0 \), define 
\begin{EQA}
	\thetavsGP
	& \eqdef &
	\argmax_{\thetav} \E L_{\GP}(\thetav) .
\label{tsGatELGt}
\end{EQA}
We use the following decomposition
\begin{EQA}
	L_{\GP}(\tilde{\thetav}_{\GP})
	&=&
	L_{\GP}(\tilde{\thetav}_{\GP}) - L_{\GP}(\thetavsGP)
	+ \E L_{\GP}(\thetavsGP) 
	+ L_{\GP}(\thetavsGP) - \E L_{\GP}(\thetavsGP).
\label{LGttGLGttGELL}
\end{EQA}
We begin by studying the first term.
 
\begin{lemma}
\label{LELGtEfs}
Let \( \epsv = \Yv - \E \Yv \) and \( \xivGP = \sigma^{-2} \DPGP^{-1} \Psi \epsv \).
Then
\begin{EQA}
	L_{\GP}(\tilde{\thetav}_{\GP}) - L_{\GP}(\thetavsGP)
	&=&
	\frac{1}{2} \bigl\| \xivGP \bigr\|^{2} .
\label{LGttGmLGtsG12}
\end{EQA}
%\begin{EQA}
%	\xivGP 
%	&=& 
%	\sigma^{-2} \DPGP^{-1} \Psi \epsv
%	=
%	\sigma^{-1} \bigl( \Psi \Psi^{\T} + \sigma^{2} \GP^{2} \bigr)^{-1} \Psi \epsv .
%\label{sm1m2Dm1LGts}
%\end{EQA} 
Moreover, if noise \( \epsv \) is homogeneous and correctly specified with 
\( \Var(\epsv) = \sigma^{2} \Id_{n} \), then
\begin{EQA}
	\E \| \xivGP \|^{2}
	&=&
	\tr \bigl( \DPc^{2} \DPGP^{-2} \bigr)
	=
	\dimA_{\GP} \, .
\label{ExG2trD2m2}
\end{EQA}
If \( \epsv \) is Gaussian then 
%\( \| \xivGP \|^{2} \) concentrates around its expectation
\begin{EQA}
	\P\Bigl( 
		\bigl| \| \xivGP \|^{2} - \E \| \xivGP \|^{2} \bigr| 
		> 2 \vA_{\GP} \sqrt{\xx} + 2\xx 
	\Bigr)
	& \leq &
	\ex^{-\xx} 
\label{exPxGExG22}
\end{EQA}
with \( \vA_{\GP}^{2} = \tr \bigl( \DPc^{2} \DPGP^{-2} \bigr)^{2} \).
\end{lemma}

\begin{proof}
The expression \( L_{\GP}(\thetav) \) is quadratic in \( \thetav \).
Moreover, \( \nabla^{2} L_{\GP}(\thetav) = - \DP_{\GP}^{2} \).
By Taylor expansion of the second order at the extremal point 
\( \tilde{\thetav}_{\GP} = \argmax_{\thetav} L_{\GP}(\thetav) \),
it holds for any \( \thetav \)
\begin{EQA}
	L_{\GP}(\tilde{\thetav}_{\GP}) - L_{\GP}(\thetav)
	&=&
	\frac{1}{2} \bigl\| \DP_{\GP} (\tilde{\thetav}_{\GP} - \thetav) \bigr\|^{2} .
\label{LGGLGttst12DGt}
\end{EQA}
This identity applied to \( \thetav = \thetavs_{\GP} = \sigma^{-2} \DP_{\GP}^{-2} \Psi \fvs \) yields \eqref{LGttGmLGtsG12}
in view of \( \E \tilde{\thetav}_{\GP} = \thetavs_{\GP} \).
The concentration bound \eqref{exPxGExG22} follows from Corollary~\ref{Cchi2p}.
\end{proof}

Theorem~\ref{LLbrevelocroB} allows to extend the bound \eqref{exPxGExG22} to
the case of arbitrary noise under exponential moment conditions. 

Now we consider the term \( \E L_{\GP}(\thetavsGP) \).

\begin{lemma}
\label{LELGTts}
Let \( \E \Yv = \fvs = \Psi^{\T} \thetavs \). 
Then with \( \Pi_{\GP} = \Psi^{\T} \bigl( \Psi \Psi^{\T} + \sigma^{2} \GP^{2} \bigr)^{-1} \Psi \), it holds
\begin{EQA}
	\thetavsGP
	& = &
	\sigma^{-2} \DPGP^{-2} \Psi \fvs 
	=
	(\Psi \Psi^{\T} + \sigma^{2} \GP^{2})^{-1} \Psi \fvs ,
	\\
	\fvs_{\GP}
	& \eqdef &
	\Psi^{\T} \thetavsGP
	=
	\Pi_{\GP} \fvs .
\label{PPTsm2G2m1Ps}
\end{EQA}
Moreover, 
\begin{EQA}
	\E L_{\GP}(\thetavsGP)
	&=&
%	- \frac{1}{2 \sigma^{2}} \bigl( \| \fvs - \Pi_{\GP} \fvs \|^{2} + \E \| \epsv \|^{2} \bigr) 
%	- \frac{1}{2} \bigl\| \GP \thetavsGP \bigr\|^{2} 
%	=
	- \frac{\bias_{\GP}^{2}}{2} - \frac{\E \| \epsv \|^{2}}{2 \sigma^{2}}  
\label{fG22Ee22s2}
\end{EQA}
with 
%\( \bias_{\GP}^{2} \eqdef \sigma^{-2} \| \fvs - \Pi_{\GP} \fvs \|^{2} + \bigl\| \GP \thetavsGP \bigr\|^{2} \).
\begin{EQA}
	\bias_{\GP}^{2}
	& \eqdef &
	\sigma^{-2} \| \fvs - \Pi_{\GP} \fvs \|^{2} + \bigl\| \GP \thetavsGP \bigr\|^{2} 
	=
	\sigma^{-2} \bigl\langle \fvs, (\Id - \Pi_{\GP}) \fvs \bigr\rangle .
\label{biG2sm2fsmPms}
\end{EQA}
%with \( \zeta_{\GP} \) from  \eqref{12s2Ee22lrf}.
\end{lemma}

\begin{proof}
The first three identities follow directly from definitions in a standard way. 
The expression \eqref{biG2sm2fsmPms} for the squared bias is obtained as follows:
\begin{EQA}
	\| \fvs - \Pi_{\GP} \fvs \|^{2} + \sigma^{2} \bigl\| \GP \thetavsGP \bigr\|^{2}
	&=&
	\| (\Id - \Pi_{\GP}) \fvs \|^{2} 
	+ \bigl\langle \thetavsGP, (\Psi \Psi^{\T} + \sigma^{2} \GP^{2} - \Psi \Psi^{\T}) \thetavsGP \bigr\rangle
	\\
	&=&
	\| (\Id - \Pi_{\GP}) \fvs \|^{2} 
	+ \bigl\langle (\Psi \Psi^{\T} + \sigma^{2} \GP^{2})^{-1} \Psi \fvs, \Psi \fvs \bigr\rangle
	- \| \Pi_{\GP} \fvs \|^{2}
	\\
	&=&
	\bigl\langle \fvs, (\Id - \Pi_{\GP}) \fvs \bigr\rangle
\label{fPiGfIPiGf}
\end{EQA}
as required.
\end{proof}


\begin{lemma}
\label{Lstochpost}
Suppose that \( \Var(\Yv) = \Var(\epsv) = \sigma^{2} \Id_{n} \).
Then
\begin{EQA}
	\E \Bigl| \sigma^{-2} \bigl\langle \epsv, \fvs - \Pi_{\GP} \fvs \bigr\rangle 
	\Bigr|^{2}
	& = &
	\sigma^{-2} \| \fvs - \Pi_{\GP} \fvs \|^{2}
	\leq 
	\bias_{\GP}^{2} .
\label{EBsm2efPiGbG2}
\end{EQA}
Moreover, if \( \epsv \sim \ND(0,\sigma^{2} \Id_{n}) \), then
on a set \( \Omega(\xx) \) of probability at least \( 1 - \ex^{-\xx} \),
it holds 
\begin{EQA}[c]
	\bigl| \sigma^{-2} \bigl\langle \epsv, \fvs - \Pi_{\GP} \fvs \bigr\rangle \bigr|
	\leq 
	\bias_{\GP} \sqrt{2\xx} \, .
\label{bGsx2vAsm2ef}
\end{EQA}
\end{lemma}


The result can be extended to non-Gaussian and misspecified noise under exponential moments 
of \( \epsv \). 
An important remark is that the term \( \| \xivGP \|^{2} \) only depends on the noise and the signal 
\( \fvs = \E \Yv \) does not  show up here.

The stochastic term \( L_{\GP}(\thetavsGP) - \E L_{\GP}(\thetavsGP) \) can be decomposed as
\begin{EQA}
	L_{\GP}(\thetavsGP) - \E L_{\GP}(\thetavsGP)
	&=&
%	L(\thetavsGP) - \E L(\thetavsGP)
%	=
%	\\
%	&=&
	\frac{1}{2 \sigma^{2}} 
	\Bigl( \E \| \epsv \|^{2} - \| \epsv \|^{2} 
		- 2 \bigl\langle \epsv, \fvs - \Pi_{\GP} \fvs \bigr\rangle 
	\Bigr) .
\label{LGmELG12s2Ee22lrf}
\end{EQA}
%
One can see that the signal \( \fvs \) or, more precisely, the bias \( \fvs - \Pi_{\GP} \fvs \) plays the leading role in the expression for \( L_{\GP}(\thetavsGP) \) and its expectation
\( \E L_{\GP}(\thetavsGP) \).
The terms \( \E \| \epsv \|^{2} \) and \( \E \| \epsv \|^{2} - \| \epsv \|^{2} \) can be large but it only depends on the noise, 
the signal \( \fvs \) or the matrix \( \GP^{2} \) do not enter there.  


We also study the relation between the values \( \penm_{\GP} \) from \eqref{cGaeldGadDGa} and 
\( \dimA_{\GP} \).
By definition \( \DPGP^{2} = \DPc^{2} + \GP^{2} \) and
\begin{EQA}
	\penm_{\GP} - \dimA_{\GP}
	&=&
	\frac{1}{2} \Bigl\{ \log \det \bigl( \Id - \DPGP^{-1} \DPc^{2} \DPGP^{-1} \bigr) 
	- \tr \bigl( \DPGP^{-1} \DPc^{2} \DPGP^{-1} \bigr) \Bigr\} .
\label{pmGpG12ldIDGm1}
\end{EQA}
Suppose without loss of generality that 
\( \DPc^{2} = \sigma^{-2} \Psi \Psi^{\T} = n \sigma^{-2} \Id_{\dimp}  \)
while \( \GP^{2} = \diag\bigl\{ \gp_{1}^{2} \leq \gp_{2}^{2} \leq \ldots \bigr\} \).
Then
\begin{EQA}
	\varA_{\GP}^{2}
	=
	\penm_{\GP} - \dimA_{\GP}
	&=&
	\frac{1}{2} \sum_{j} - \log\Bigl( 1 - \frac{n \sigma^{-2}}{n \sigma^{-2} + \gp_{j}^{2}} \Bigr)
	- \frac{n \sigma^{-2}}{n \sigma^{-2} + \gp_{j}^{2}} \, .
\label{vAG2pGpG12sm2}
\end{EQA}
We use that \( - \log(1 - \xx) - \xx \geq \xx^{2}/2 \) yielding 
\begin{EQA}
	\penm_{\GP} - \dimA_{\GP}
	& \geq &
	\frac{1}{2} \tr\bigl( \DPGP^{-1} \DPc^{2} \DPGP^{-1} \bigr)^{2} .
\label{pmGmpG12tDGm12m122}
\end{EQA}
This completes the proof of \eqref{2efPf22x2Ex2}. 
\end{proof}

Putting together the representation \eqref{hcYcGapGaLGa1} and the decomposition \eqref{2efPf22x2Ex2} yields 
the result of the theorem. 



\subsection{Proof of Theorem~\ref{Tpostcontpr}}
For each \( \hyper \in \MMd_{\priorh} \), fix 
\( \hypers = \hypers(\hyper) \in \MMs_{\priorh} \) such that 
\( \riskt_{\hyper} - \riskt_{\hypers} > \disth(\hyper,\hypers) \).
It follows from the representation \eqref{hcYcGapGaLGa22} in an obvious way 
that the posterior probability of the set \( \MMd_{\priorh} \) satisfies 
\begin{EQA}
	\priorh(\MMd_{\priorh},\Yv)
	& \leq &
	\sum_{\hyper \in \MMd_{\priorh}} 
		\exp\bigl( \risktt_{\hypers} - \risktt_{\hyper} \bigr) 
	=
	\sum_{\hyper \in \MMd_{\priorh}} 
		\exp\bigl( \riskt_{\hypers} - \riskt_{\hyper} - \zeta_{\hyper} + \zeta_{\hypers} \bigr)	
\label{pMdpYMdtrkks}
\end{EQA}
with
\begin{EQA}
	\zeta_{\hyper} - \zeta_{\hypers}
	&=&
	\frac{1}{2} \Bigl\{ \bigl( \| \xiv_{\hyper} \|^{2} - \| \xiv_{\hypers} \|^{2} \bigr) - \E \bigl( \| \xiv_{\hyper} \|^{2} - \| \xiv_{\hypers} \|^{2} \bigr) 
	\Bigr\}
	+ \sigma^{-2} \bigl\langle \epsv, \bigl( \Pi_{\hyper} - \Pi_{\hypers} \bigr) \fvs 
	\bigr\rangle \, 
\label{sm2PikPis12zzks}
\end{EQA}
and \( \xiv_{\hyper} = \sigma^{-1} \DP_{\hyper}^{-1} \Psi \epsv \).
For each \( \hyper \) from this sum, 
\begin{EQA}
	\| \xiv_{\hyper} \|^{2} - \| \xiv_{\hypers} \|^{2}
	&=&
	\sigma^{-2} \bigl\langle  
		\Psi^{\T}\bigl( \DP_{\hyper}^{-2} - \DP_{\hypers}^{-2} \bigr) 
		\Psi \epsv,  \epsv \rangle
\label{Psim2Dmm2sm2}
\end{EQA}
and by Theorem~\ref{TexpbLGA}, it holds with probability at least 
\( 1 - 2 \ex^{-\xx} \) that
\begin{EQA}
	\Bigl| \| \xiv_{\hyper} \|^{2} - \| \xiv_{\hypers} \|^{2} \Bigr|
	& \leq &
	2 \vA_{\hyper,\hypers} \sqrt{\xx} + 2 \lambda_{\hyper,\hypers} \, \xx
\label{2vkkssx2x}
\end{EQA}
where \( \vA_{\hyper,\hypers}^{2} \) and \( \lambda_{\hyper,\hypers} \) are given in \eqref{bikk2vakk222}.
%\begin{EQA}
%	\vA_{\hyper,\hypers}^{2}
%	&=&
%	\tr \Bigl\{ \DPc^{2} \bigl( \DP_{\hyper}^{-2} - \DP_{\hypers}^{-2} \bigr) \Bigr\}^{2} .
%\label{bikk2vakk2}
%\end{EQA}
Also \( \eta = \sigma^{-2} \bigl\langle \epsv, \bigl( \Pi_{\hyper} - \Pi_{\hypers} \bigr) \fvs \bigr\rangle \) is normal zero mean with the variance 
\begin{EQA}
	\Var(\eta)
	=
	\sigma^{-2} \bigl\| \bigl( \Pi_{\hyper} - \Pi_{\hypers} \bigr) \fvs \bigr\|^{2} 
	& \leq &
	\sigma^{-2} \bigl| \bigl\langle \fvs, (\Pi_{\hyper} - \Pi_{\hypers}) \fvs \bigr\rangle \bigr|
	=
	\bias_{\hyper,\hypers}^{2} .
\label{b2kkssm2m2}
\end{EQA}
Therefore, \( \P(|\eta| > \bias_{\hyper,\hypers} \sqrt{2\xx} \, ) \leq \ex^{-\xx} \)
and it holds on a random set 
\( \Omega_{\hyper}(\xx) \) with \( \P\bigl( \Omega_{\hyper}(\xx) \bigr) \geq 1 - 3 \ex^{-\xx} \) 
\begin{EQA}
	\bigl| \zeta_{\hyper,\hypers} \bigr|
	& \leq & 
	\bias_{\hyper,\hypers} \sqrt{2\xx} + \vA_{\hyper,\hypers} \sqrt{\xx} 
	+ \lambda_{\hyper,\hypers} \, \xx .
\label{bkk2sx2xvavAsx}
\end{EQA}
This implies by \eqref{dks2xbksvkssx} that on \( \Omega_{\hyper}(\xx) \)
\begin{EQA}
	\risktt_{\hypers} - \risktt_{\hyper}
	& \leq &
	\riskt_{\hypers} - \riskt_{\hyper} + \disth(\hyper,\hypers) 
	\leq 
	- \xx .
\label{rttrtsrkrsdksmx}
\end{EQA}
Similar bounds hold for each \( \hyper \in \MMd_{\priorh} \) and 
thus, on the set \( \Omega(\xx) = \bigcap_{\hyper} \Omega_{\hyper}(\xx) \)
of probability at least \( 1 - 3 |\MM| \ex^{-\xx} \), we obtain
\begin{EQA}
	\priorh(\MMd_{\priorh},\Yv)
	& \leq &
	\sum_{\hyper \in \MMd_{\priorh}} 
		\exp\bigl\{ \riskt_{\hypers} - \riskt_{\hyper} + \disth(\hyper,\hypers \bigr)
		\bigr\}
	\leq 
	|\MM| \ex^{-\xx}
\label{pMdpYMdtrkksMMex}
\end{EQA}
and \eqref{MexEpMdsYdks} follows. 


==> A_qf_shortm.tex <==
% !TEX root = ../pa_np_bvm.tex
\def\Eg{\E_{\gammav}}
\def\Pg{\P_{\gammav}}
\def\Eg{\E_{\gammav \sim \ND(0,\Id)}}
\def\Pg{\P_{\gammav \sim \ND(0,\Id)}}
\def\HPi{\QP}
\subsection{Deviation bounds for Gaussian quadratic forms}
\label{SdevboundGauss}
The next result explains the concentration effect of 
\( \langle \BB \gaussv, \gaussv \rangle \)
for a standard Gaussian vector \( \gaussv \) and a symmetric trace operator \( \BB \) in \( \R^{\dimp} \),
\( \dimp \leq \infty \).
We use a version from \cite{laurentmassart2000}.


\begin{theorem}
\label{TexpbLGA}
\label{Lxiv2LD}
\label{Cuvepsuv0}
Let \( \gaussv \) be a standard normal Gaussian element in \( \R^{\dimp} \) and \( \BB \) be symmetric non-negative trace operator in \( \R^{\dimp} \).
Then with \( \dimA = \tr(\BB) \), \( \vA^{2} = \tr(\BB^{2}) \), and 
\( \supA = \| \BB \|_{\oper} \), it holds for each \( \xx \geq 0 \)
\begin{EQA}
\label{Pxiv2dimAvp12}
	&&
	\P\Bigl( \langle \BB \gaussv, \gaussv \rangle > \zq^{2}(\BB,\xx) \Bigr)
	\leq
	\ex^{-\xx} ,
	\\
	&& \zq(\BB,\xx)
	\eqdef
	\sqrt{\dimA + 2 \vA \xx^{1/2} + 2 \supA \xx} \,\, .
\label{zqdefGQF}
\end{EQA}
In particular, it implies 
\begin{EQA}
	\P\bigl( \| \BB^{1/2} \gaussv \| > \dimA^{1/2} + (2 \supA \xx)^{1/2} \bigr)
	& \leq &
	\ex^{-\xx} .
\label{Pxiv2dimAxx12}
\end{EQA}
Also
\begin{EQA}
	\P\bigl( \langle \BB \gaussv, \gaussv \rangle < \dimA - 2 \vA \xx^{1/2} \bigr)
	& \leq &
	\ex^{-\xx} .
\label{Pxiv2dimAvp12m}
\end{EQA}
%
If \( \BB \) is symmetric but non necessarily positive then
\begin{EQA}
	\P\bigl( \bigl| \langle \BB \gaussv, \gaussv \rangle - \dimA \bigr| > 2 \vA \xx^{1/2} + 2 \supA \xx \bigr)
	& \leq &
	2 \ex^{-\xx} .
\label{PxivTBBdimA2vp}
\end{EQA}
\end{theorem}

\begin{proof}
W.l.o.g. assume \( \supA = \| \BB \|_{\infty} = 1 \).
We apply the exponential Chebyshev inequality: with \( \mu > 0 \)
\begin{EQA}
	\P\Bigl( \langle \BB \gaussv, \gaussv \rangle > \zq^{2} \Bigr)
	& \leq &
	\E \exp \Bigl( \mu \langle \BB \gaussv, \gaussv \rangle / 2 - \mu \zq^{2} / 2 \Bigr) \, .
\label{PBggiz2E2mz2}
\end{EQA}
Given \( \xx > 0 \), fix \( \mu < 1 \) by the equation
\begin{EQA}
	\frac{\mu}{1 - \mu} 
	&=&
	\frac{2 \sqrt{\xx}}{\vA} \, 
	\quad \text{ or } \quad
	\mu^{-1} 
	=
	1 + \frac{\vA}{2 \sqrt{\xx}} \, .
\label{1v2sxm12m1m}
\end{EQA}
Let \( \lambda_{j} \) be ordered eigenvalues of \( \BB \), 
\( 1 = \lambda_{1} \geq \lambda_{2} \geq \lambda_{3} \ldots \).
It holds with \( \dimA = \tr \BB \)
\begin{EQA}
	&& \nquad
	\log \E \Bigl\{ \frac{\mu}{2} \bigl( \langle \BB \gaussv, \gaussv \rangle - \dimA \bigr) \Bigr\}
	=
	\log \det(\Id - \mu \BB)^{-1/2} - \frac{\mu \, \dimA}{2}
	=
	- \frac{1}{2} \sum_{j \leq \dimp} \bigl\{ \log(1 - \mu \lambda_{j}) + \mu \lambda_{j} \bigr\}
	\\
	&=&
	\frac{1}{2} \sum_{j=1}^{\dimp} \sum_{k=2}^{\infty} \frac{(\mu \lambda_{j})^{k}}{k}
	\leq 
	\sum_{j=1}^{\dimp} \frac{(\mu \lambda_{j})^{2}}{4} \sum_{k=0}^{\infty} (\mu \lambda_{j})^{k}
	\leq 
	\sum_{j=1}^{\dimp} \frac{\mu^{2} \lambda_{j}^{2}}{4 (1 - \mu)} 
	=
	\frac{\mu^{2} \vA^{2}}{4 (1 - \mu)} \, .
\label{m2v241m4mj1p}
\end{EQA}
It remains to check that the choice \( \mu \) by \eqref{1v2sxm12m1m} and 
\( \zq = \zq(\BB,\xx) \) yields
\begin{EQA}
	\frac{\mu^{2} \vA^{2}}{4 (1 - \mu)} - \frac{\mu (\zq^{2} - \dimA)}{2}
	& = &
	\frac{\mu^{2} \vA^{2}}{4 (1 - \mu)} - \mu \bigl( \vA \sqrt{\xx} + \xx \bigr)
	=
	\mu \Bigl\{ \frac{\vA \sqrt{\xx}}{2} - \vA \sqrt{\xx} - \xx \Bigr\}
	=
	- \xx
	\qquad
	\qquad
\label{m2vA241muz2}
\end{EQA}
as required.
\end{proof}
As a special case, we present a bound for the chi-squared distribution 
corresponding to \( \BB = \Id_{\dimp} \), \( \dimp < \infty \).
Then \( \tr (\BB) = \dimp \), \( \tr(\BB^{2}) = \dimp \) and \( \supA(\BB) = 1 \).

\begin{corollary}
\label{Cchi2p}
Let \( \gaussv \) be a standard normal vector in \( \R^{\dimp} \).
Then for any \( \xx > 0 \)
\begin{EQA}[ccl]
\label{Pxi2pm2px}
	\P\bigl( \| \gaussv \|^{2} \geq \dimp + 2 \sqrt{\dimp \xx} + 2 \xx \bigr)
	& \leq &
	\ex^{-\xx},
	\\
	\P\bigl( \| \gaussv \| \,\,  \geq \sqrt{\dimp} + \sqrt{2 \xx} \bigr)
	& \leq &
	\ex^{-\xx} ,
\label{Pxi2pm2px12}
	\\
	\P\bigl( \| \gaussv \|^{2} \leq \dimp - 2 \sqrt{\dimp \xx} \bigr)
	& \leq &
	\ex^{-\xx}	.
\label{Pxi2pm2px22}
\end{EQA}
\end{corollary}

%Finally we bound an expectation of the exponent \( \exp(\bv^{\T} \gaussv) \)
%over the set \( \gaussv^{\T} \BB \gaussv > \zq^{2}(\BB,\xx) \). 
%
%\begin{theorem}
%\label{TexpindqfG}
%Let \( \BB \) be symmetric non-negative \( \dimp \)-matrix with \( \| \BB \| \leq 1 \) 
%and let \( \gammav \) be standard normal in \( \R^{\dimp} \).
%For any \( \xx > 0 \) and a vector \( \bv \in \R^{\dimp} \), it holds with 
%\( \zq^{2}(\BB,\xx) \) from \eqref{zqdefGQF}
%\begin{EQA}
%	\E \exp\bigl( \bv^{\T} \gaussv \bigr)
%	 	\Ind\bigl( \gaussv^{\T} \BB \gaussv > \zq^{2}(\BB,\xx) \bigr)
%	& \leq &
%	\exp\bigl( - \xx + \bigl( 1 + 2 \xx^{1/2}/\vA \bigr) \| \bv \|^{2} \bigr) .
%\label{EbvTgIgTB12}
%\end{EQA}
%\end{theorem}
%\begin{proof}
%For any \( \mu \in (0,1) \), it holds
%\begin{EQA}
%	\E \exp\bigl( \bv^{\T} \gaussv \bigr)
%	 	\Ind\bigl( \gaussv^{\T} \BB \gaussv > \zq^{2}(\BB,\xx) \bigr)
%	& \leq &
%	\E \exp\Bigl( \bv^{\T} \gaussv + \mu \bigl\{ \gaussv^{\T} \BB \gaussv - \zq^{2}(\BB,\xx) \bigr\} \Bigr)
%\label{BxbTgmuz2}
%\end{EQA}
%Further, by the change of variables,
%\begin{EQA}
%	&& \nquad
%	\E \exp\Bigl( 
%		\bv^{\T} \gaussv 
%		+ \mu \bigl\{ \gaussv^{\T} \BB \gaussv - \zq^{2}(\BB,\xx) \bigr\} 
%	\Bigr)
%	\\
%	&=&
%	\exp\bigl( \bv^{\T} (\Id - \mu \BB)^{-1} \bv / 2 \bigr)
%	\E \exp\Bigl( 
%		\mu \bigl\{ \gaussv^{\T} \BB \gaussv - \zq^{2}(\BB,\xx) \bigr\} 
%	\Bigr) .
%\label{EbTImuBm12z2}
%\end{EQA}
%The choice \( \mu = \xx^{1/2}/ \bigl( \xx^{1/2} + \vA/2 \bigr) \) yields
%\begin{EQA}
%	\E \exp\Bigl( 
%		\mu \bigl\{ \gaussv^{\T} \BB \gaussv - \zq^{2}(\BB,\xx) \bigr\} 
%	\Bigr)
%	& \leq &
%	\ex^{-\xx} ;
%\label{exv2x12b2}
%\end{EQA}
%see the proof of Theorem~\ref{TexpbLGA}.
%Moreover, 
%in view of \( \| \BB \|_{\oper} \leq 1 \), it holds
%\begin{EQA}
%	\bv^{\T} (\Id - \mu \BB)^{-1} \bv
%	& \leq &
%	\frac{\vA + 2 \xx^{1/2}}{\vA} \| \bv \|^{2} .
%\label{bTbImuBbv212}
%\end{EQA}
%This implies the first assertion.
%
%By the Cauchy-Schwarz inequality 
%\begin{EQA}
%	\E \exp\bigl( \bv^{\T} \gaussv \bigr)
%	 	\Ind\bigl( \gaussv^{\T} \BB \gaussv > \zq^{2}(\BB,\xx) \bigr)
%	& \leq &
%	\sqrt{\E \exp\bigl( 2 \bv^{\T} \gaussv \bigr) 
%	\P\bigl( \gaussv^{\T} \BB \gaussv > \zq^{2}(\BB,\xx) \bigr)} 
%	\\
%	& \leq &
%	\exp\bigl( 2 \| \bv \|^{2} - \xx/2 \bigr) .
%\label{EbvTgIgTB222}
%\end{EQA}
%Let now \( \gaussv^{\T} \BB \gaussv = \| \AA \gaussv \|^{2} \).
%For a fixed \( \rr \),
%\begin{EQA}
%	\E \exp\bigl( \bv^{\T} \gaussv \bigr)
%	 	\Ind\bigl( \| \AA \gaussv \| > \rr \bigr)
%	& = &
%	\frac{1}{(2\pi)^{\dimp/2}} \int \exp\Bigl( \bv^{\T} \gaussv - \frac{\| \gaussv \|^{2}}{2} \Bigr)
%	 	\Ind\bigl( \| \AA \gaussv \| > \rr \bigr) d \gaussv
%	\\
%	&=&
%	\frac{\ex^{\| \bv \|^{2}/2}}{(2\pi)^{\dimp/2}} 
%	\int \exp\Bigl( - \frac{\| \gaussv - \bv \|^{2}}{2} \Bigr)
%	 	\Ind\bigl( \| \AA \gaussv \| > \rr \bigr) d \gaussv
%	\\
%	&=&
%	\ex^{\| \bv \|^{2}/2} \P\bigl( \| \AA (\gaussv + \bv) \| > \rr  \bigr)
%	\\
%	& \leq &
%	\ex^{\| \bv \|^{2}/2} \P\bigl( \| \AA \gaussv \| > \rr - \| \AA \bv \| \bigr)
%\label{•}
%\end{EQA}
%\end{proof}
%


\subsection{Deviation bounds for non-Gaussian quadratic forms}
\label{Sprobabquad}
\label{SdevboundnonGauss}
This section collects some probability bounds for non-Gaussian quadratic forms.
The presented results can be viewed as a slight improvement of the bounds from \cite{SP2011}.
%  using the deviation bound from \cite{laurentmassart2000}.
%The proofs are very similar to ones from \cite{SP2011} and are omitted by the space reasons. 
%For the rigorous proofs we refer to the supplementary paper \cite{SP2013_rough}.
%\Section{Deviation bounds for non-Gaussian quadratic forms}

Let \( \xiv \) be a random vector in \( \R^{\dimp} \), \( \dimp \leq \infty \)
satisfying for some fixed \( \gmb > 0 \)  
\begin{EQA}[c]
    \log \E \exp\bigl( \langle \uv, \xiv \rangle \bigr)
    \le
    \| \uv \|^{2}/2,
    \qquad
    \uv \in \R^{\dimp}, \, \| \HPc \uv \| \le \gmb ,
\label{expgamgme}
\end{EQA}
for some self-adjoint operator \( \HPc \) in \( \R^{\dimp} \), \( \HPc \geq \Id_{\dimp} \).
In fact, it suffices to assume that 
\begin{EQA}
	\sup_{\| \HPc \uv \| \leq \gmb} \E \exp\bigl( \langle \uv, \xiv \rangle \bigr)
	& \leq &
	\CONST .
\label{sgagEexlgHx}
\end{EQA}
Then one can use the fact that existence of the exponential moment \( \E \ex^{\lambda_{0} \xi} \) for a centered random variable \( \xi \) and some fixed \( \lambda_{0} \) implies that the moment generating function 
\( f_{\xi}(\lambda) \eqdef \log \E \ex^{\lambda \xi} \) is analytic in \( \lambda \in (0, \lambda_{0}) \) with 
\( f_{\xi}(0) = f'_{\xi}(0) = 0 \) and hence, it can be well majorated by a quadratic function in a smaller interval 
\( [0,\lambda_{1}] \) for \( \lambda_{1} < \lambda_{0} \); see~\cite{GolSpo2009}.

%
We present a bound for a quadratic form \( \langle \BB \xiv, \xiv \rangle \), where 
\( \xiv \) satisfies \eqref{expgamgme} and \( \BB \) is a given symmetric non-negative 
operator in \( \R^{\dimp} \) such that \( \BB \leq \HPc^{-2} \) and
\( \HPc \BB \HPc \) is a trace operator:
\begin{EQA}
	\dimA_{\HPc}
	&=&
	\tr\bigl( \HPc^{2} \BB \bigr) 
	< \infty.
\label{dimAtHm2Bpp}
\end{EQA}
By normalization, one can easily reduce the study to the case with 
\begin{EQA}
	\| \BB \|
	&=&
	1 .
\label{BBeq1qgnG}
\end{EQA}
Denote
\begin{EQA}[c]
    \dimB
    \eqdef
    \tr \bigl( \BB \bigr) ,
    \qquad 
    \vpB^{2}
    \eqdef
    \tr(\BB^{2}) .
%    \qquad
%    \lambdaB \eqdef \lambda_{\max}\bigl( \BB \bigr). 
\label{BBrddB}
\end{EQA}   
We show that under these conditions, the quadratic form \( \langle \BB \xiv, \xiv \rangle \)
follows essentially the same deviation bound 
\( \P\bigl( \langle \BB \xiv, \xiv \rangle \ge \zq^{2}(\BB,\xx) \bigr) \lesssim \ex^{-\xx} \) 
with \( \zq^{2}(\BB,\xx) = \dimA + 2 \vp \xx^{1/2} + 2 \xx \)
as in the Gaussian case.
Let \( \mu(\xx) \) be defined by \( \mu(\xx) = \bigl( 1 + \frac{\vA}{2 \sqrt{\xx}} \bigr)^{-1} \);
see \eqref{1v2sxm12m1m}. 
Obviously \( \mu(\xx) \) grows with \( \xx \).
Define the value \( \xxc \) by the equation
\begin{EQA}
	\frac{\gmb - \sqrt{\dimA_{\HPc} \, \mu(\xxc)}}{\mu(\xxc)} 
	& = &
	\zq(\BB,\xxc) + 1 .
\label{gmsqpAHmxzBx1}
\end{EQA}
Also denote \( \muc = \mu(\xxc) \) and
\begin{EQA}
	\gmc
	&=&
	\gmb - \sqrt{\dimA_{\HPc} \muc} \, .
\label{gcgbsqpHmc}
\end{EQA}
Obviously \( \gmb - \sqrt{\dimA_{\HPc}} \leq \gmc \leq \gmb \).
Moreover, as \( \zq(\BB,\xx) \leq \sqrt{\dimA} + \sqrt{2 \xx} \), we derive that 
\begin{EQA}
	\sqrt{2\xxc}
	& \geq &
	\gmc/\muc - \sqrt{\dimA} \, .
\label{sxcgbspHspA}
\end{EQA}
Our results implicitly assume that \( \xxc \) is large, that is, 
\( \gmb \gg \sqrt{\dimA_{\HPc}} + \sqrt{\dimA} \). 

\begin{theorem}
\label{LLbrevelocroB}   
Let \eqref{expgamgme} hold and let \( \BB \) be such that, \( \| \BB \| = 1 \)
%, \( \BB \leq \HPc^{-2} \) 
and moreover, \( \dimA_{\HPc} = \tr(\HPc^{2} \BB) < \infty \).
Define \( \xxc \) by \eqref{gmsqpAHmxzBx1} and \( \gmc \) by \eqref{gcgbsqpHmc}, and suppose
\( \gmc \geq 1 \).
Then for any \( \xx > 0 \)
\begin{EQA}
    \P\bigl( \langle \BB \xiv, \xiv \rangle \ge \zqc^{2}(\BB,\xx) \bigr)
    & \le &
    2 \ex^{-\xx} + \ex^{-\xxc} \Ind(\xx < \xxc) ,
\label{PxivbzzBBroB}
\end{EQA}    
where \( \zqc(\BB,\xx) \) is defined by
\begin{EQA}
\label{PzzxxpBroB}
    \zqc(\BB,\xx)
    & \eqdef &
    \begin{cases}
      \sqrt{ \dimA + 2 \vp \xx^{1/2} + 2 \xx } \, , &  \xx \le \xxc \,, 
      \\
      \gmc/\muc + 2 (\xx - \xxc)/\gmc \, , & \xx > \xxc \, .
    \end{cases}
\label{zzxxppdBlroB}
\end{EQA}    
If \eqref{expgamgm} hold with \( \gm = \infty \), then
\begin{EQA}
    \P\bigl( \langle \BB \xiv, \xiv \rangle \ge \zq^{2}(\BB,\xx) \bigr)
    & \le &
    \ex^{-\xx}  ,
    \quad
    \zq^{2}(\BB,\xx)
    =
    \dimA + 2 \vp \xx^{1/2} + 2 \supA \xx  \, .
%    \leq 
%    \sqrt{\dimA} + \sqrt{2 \supA \xx} \, .
\label{PxivbzzBBroBinf}
\end{EQA}    
\end{theorem}

The value 
\( \zq(\BB,\xx) = \sqrt{ \dimA + 2 \vp \xx^{1/2} + 2 \xx } \) can be upper bounded 
by \( \sqrt{\dimA} + \sqrt{2 \xx} \):
\begin{EQA}
\label{PzzxxpBroBu}
    \zqc(\BB,\xx)
    & \leq &
    \begin{cases}
        \sqrt{\dimA} + \sqrt{2 \xx}, &  \xx \le \xxc, \\
        \zqc + 2 (\xx - \xxc)/\gmc , & \xx > \xxc.
    \end{cases}
\end{EQA}    

Depending on the value \( \xx \), we have two types of tail behavior of the 
quadratic form \( \| \xiv \|^{2} \). 
For \( \xx \le \xxc \), we have essentially the same deviation bounds as in the Gaussian case
with the extra-factor two in the deviation probability.
For \( \xx > \xxc \), we switch to the special regime driven by the exponential moment
condition \eqref{expgamgm}.
Usually \( \gmb^{2} \) is a large number (of order \( n \) in the i.i.d. setup) and 
the second term in \eqref{PxivbzzBBro} can be simply ignored. 
The sub-Gaussian case with \( \gmb = \infty \) leads to the same bound \eqref{Pxiv2dimAvp12}
as in the Gaussian case.

As a corollary, we state the result for the norm of \( \xiv \in \R^{\dimp} \) corresponding to the case
\( \HPc^{-2} = \BB = \Id_{\dimp} \) and \( \dimp < \infty \). 
Then 
\begin{EQA}
	\dimA
	&=&
	\dimA_{\HPc}
	=
	\vA^{2}
	=
	\dimp,
	\quad
	\lambda = 1.
\label{pApHpvA2l1}
\end{EQA}

\begin{theorem}
\label{LLbrevelocro}   
Let \eqref{expgamgm} hold with \( \HPc = \Id_{\dimp} \) and 
\( \gm > 2 \sqrt{\dimp} \).
Then for each \( \xx > 0 \)
\begin{EQA}
    \P\bigl( \| \xiv \| \ge \zqc(\dimp,\xx) \bigr)
    & \le &
    2 \ex^{-\xx} + \ex^{-\xxc } \Ind(\xx < \xxc) ,
\label{PxivbzzBBro}
\end{EQA}    
where \( \zqc(\dimp,\xx) \) is defined by
\begin{EQA}
\label{PzzxxpBro}
    \zqc(\dimp,\xx)
    & \eqdef &
    \begin{cases}
      \bigl( \dimp + 2 \sqrt{\dimp \xx} + 2 \xx\bigr)^{1/2}, &  \xx \le \xxc  , \\
      \gmc/\muc + 2 \gmc^{-1} (\xx - \xxc)   , & \xx > \xxc .
    \end{cases}
\label{zzxxppdBlro}
\end{EQA}    
\end{theorem}

\begin{remark}
The same bound \eqref{PxivbzzBBroB} applies 
for a general matrix \( \BB \) with \( \| \BB \| \leq 1 \).
%\begin{EQA}
%\label{PzzxxpBroB}
%    \zqc(\BB,\xx)
%    & \eqdef &
%    \begin{cases}
%      \sqrt{ \dimA + 2 \vp \xx^{1/2} + 2 \lambdaB \xx } \, , &  \xx \le \xxc \,, 
%      \\
%      \gmc/\muc + 2 \lambdaB (\xx - \xxc)/\gmc \, , & \xx > \xxc \, .
%    \end{cases}
%\label{zzxxppdBlroBl}
%\end{EQA}    
\end{remark}

\begin{proof}[Proof of Theorem~\ref{LLbrevelocroB}]
We will use \eqref{expgamgme} in the equavalent form
\begin{EQA}[c]
    \log \E \exp\bigl( \langle \HPc^{-1} \uv, \xiv \rangle \bigr)
    =
    \log \E \exp\bigl( \langle \uv, \HPc^{-1} \xiv \rangle \bigr)
    \le
    \| \HPc^{-1} \uv \|^{2}/2,
    \quad
    \| \uv \| \le \gmb .
    \qquad
\label{expgamgm}
\end{EQA}
%
First we consider the most interesting case \( \xx \leq \xxc \). 
We expect to get Gaussian type deviation bounds for such \( \xx \).
%For any \( \mu < 1 \), we use the identity
%\begin{EQA}
%	\exp\bigl( \mu \langle \BB \xiv, \xiv \rangle / 2 \bigr)
%	&=&
%	\Eg \exp\bigl( \mu^{1/2} \langle \HPc \BB^{1/2} \gammav, \HPi \xiv \rangle \bigr)
%\label{Egexmu12lHm1B12}
%\end{EQA}
%for a standard Gaussian \( \gammav \) and \( \Eg(\cdot) = \E\bigl( \cdot \cond \xiv \bigr) \).
%
The main tool for the proof is the following lemma.
\begin{lemma}
\label{LGDBqfexpB}
Let \( \mu \in (0,1) \) and \( \zz(\mu) = \gmb / \mu - \sqrt{\dimA_{\HPc}/\mu} > 0 \).
Then \eqref{expgamgm} implies
\begin{EQA}
	\E \exp\bigl( \mu \langle \BB \xiv, \xiv \rangle / 2 \bigr)
	\Ind\bigl( \| \HPc \BB \xiv \| \leq \zz(\mu) \bigr)
	& \leq &
	2 \exp \Bigl( \frac{\mu^{2} \vA^{2}}{4 (1 - \mu)} + \frac{\mu \tr \BB}{2} \Bigr) .
\label{wBmu2vA241mmutrB}
\end{EQA}
Moreover, if \( \gmb = \infty \), then
\begin{EQA}
	\E \exp\bigl( \mu \langle \BB \xiv, \xiv \rangle / 2 \bigr)
	& \leq &
	\exp \Bigl( \frac{\mu^{2} \vA^{2}}{4 (1 - \mu)} + \frac{\mu \tr \BB}{2} \Bigr) .
\label{wBmu2vA241mmutrBi}
\end{EQA}
\end{lemma}

\begin{proof}
Let us fix for a moment some \( \xiv \in \R^{\dimp} \) and \( \mu < 1 \) and
define 
\begin{EQA}
	\av = \HPc^{-1} \xiv, 
	&\qquad & 
	\Sigma = \mu \HPc \BB \HPc .
\label{aSigmHm1xivmuc}
\end{EQA}
Consider the Gaussian measure \( \P_{\av,\Sigma} = \ND(\av,\Sigma^{-1}) \), and 
let \( \Uv \sim \ND(0,\Sigma^{-1}) \).
By the Girsanov formula
\begin{EQA}
	\log \frac{d\P_{\av,\Sigma}}{d\P_{0,\Sigma}}(\uv)
	&=&
	\langle \Sigma \av, \uv \rangle - \frac{1}{2} \bigl\langle \Sigma \av, \av \bigr\rangle
\label{GirslogddPaSSm1}
\end{EQA}
and for any set \( A \in \R^{\dimp} \)
\begin{EQA}
	\P_{\av,\Sigma}(A)
	&=&
	\P_{0,\Sigma}(A - \av)
	=
	\E_{0,\Sigma} \Bigl[ 
		\exp\Bigl\{ \langle \Sigma \Uv, \av \rangle 
			- \frac{1}{2} \bigl\langle \Sigma \av, \av \bigr\rangle \Bigr\} \Ind(A) 
	\Bigr] .
\label{PaSAP0SAav}
\end{EQA}
Now we select \( A = \bigl\{ \uv \colon \| \Sigma \uv \| \leq \gmb \bigr\} \).
Under \( \P_{0,\Sigma} \), one can represent 
\( \Sigma \Uv = \Sigma^{1/2} \gammav 
= \mu^{1/2} \HPc \BB^{1/2} \gammav \) with a standard Gaussian 
\( \gammav \).
Therefore,
\begin{EQA}
	\P_{0,\Sigma}(A - \av)
	&=&
	\Pg\bigl( \| \Sigma^{1/2} (\gammav - \Sigma^{1/2} \av) \| \leq \gmb \bigr)
	\\
	& \geq &
	\Pg\bigl( \| \Sigma^{1/2} \gammav \| \leq \gmb - \| \Sigma \av \| \bigr) .
\label{P0SAmaPgSm12}
\end{EQA}
We now use that \( \Pg\bigl( \| \Sigma^{1/2} \gammav \|^{2} \leq \tr (\Sigma) \bigr) \geq 1/2 \)
with \( \tr(\Sigma) = \mu \tr(\HPc^{2} \BB ) = \mu \, \dimA_{\HPc} \).
Therefore, the condition \( \| \Sigma \av \| + \sqrt{\mu \, \dimA_{\HPc}} \leq \gmb \) implies
in view of \( \langle \Sigma \av, \av \rangle = \mu \langle \BB \xiv, \xiv \rangle \)
\begin{EQA}
	1/2
	\leq 
	\P_{\av,\Sigma}(A)
	&=&
	\E_{0,\Sigma} \Bigl[ 
		\exp\Bigl\{ \langle \Sigma \Uv, \HPc^{-1} \xiv \rangle
			- \mu \langle \BB \xiv, \xiv \rangle / 2 \Bigr\} 
			\Ind( \| \Sigma \Uv \| \leq \gmb) 
	\Bigr]
\label{12PavSAE0SISm1}
\end{EQA}
or
\begin{EQA}
	&& \nquad
	\exp\bigl( \mu \langle \BB \xiv, \xiv \rangle / 2 \bigr)
	\Ind\bigl( \| \Sigma \HPc^{-1} \xiv \| \leq \gmb - \sqrt{\mu \, \dimA_{\HPc}} \bigr)
	\\
	& \leq &
	2 \E_{0,\Sigma} \Bigl[ 
		\exp\Bigl\{ \langle \Sigma \Uv, \HPc^{-1} \xiv \rangle
			\Ind( \| \Sigma \Uv \| \leq \gmb) 
	\Bigr] .
\label{emNxx22E0Sm1u}
\end{EQA}
We now take the expectation of the each side of this equation w.r.t. \( \xiv \),
change the integration order, and use \eqref{expgamgm} yielding
\begin{EQA}
	&& \nquad
	\E \exp\bigl( \mu \langle \BB \xiv, \xiv \rangle / 2 \bigr)
	\Ind\bigl( \| \Sigma \HPc^{-1} \xiv \| \leq \gmb - \sqrt{\mu \, \dimA_{\HPc}} \bigr)
	\leq 
	2 \E_{0,\Sigma} \exp\bigl( \| \HPc^{-1} \Sigma \Uv \|^{2} / 2 \bigr)
	\\
	&=&
	2 \Eg \exp\bigl( \| \BB^{1/2} \gammav \|^{2} / 2 \bigr)
	=
	2 \det\bigl( \Id - \mu \BB \bigr)^{-1/2} .
%		\Ind\bigl( \| \HPc \BB^{1/2} \gammav \| \leq \gmb \bigr)
\label{IHm1B12EgEgg}
\end{EQA}
We also use that for any \( \mu > 0 \)
\begin{EQA}
	\log \det\bigl( \Id - \mu \BB \bigr)^{-1/2} - \frac{\mu \tr \BB}{2}
	& \leq &
	\frac{\mu^{2} \vA^{2}}{4 (1 - \mu)} \, ;
\label{mu2v241mmiulogIm12}
\end{EQA}
see \eqref{m2v241m4mj1p}, 
and the first statement follows in view of \( \Sigma \HPc^{-1} \xiv = \mu \HPc \BB \xiv \).

The proof of the second one is much easier. 
For any \( \mu < 1 \), we use the identity
\begin{EQA}
	\E \exp\bigl( \mu \langle \BB \xiv, \xiv \rangle / 2 \bigr)
	&=&
	\E \Eg \exp\bigl( \mu^{1/2} \langle \HPc \BB^{1/2} \gammav, \HPc^{-1} \xiv \rangle \bigr)
\label{Egexmu12lHm1B12}
\end{EQA}
%for a standard Gaussian \( \gammav \) and \( \Eg(\cdot) = \E\bigl( \cdot \cond \xiv \bigr) \).
Application of Fubini's theorem and \eqref{expgamgm} reduces the study to the Gaussian case; cf. \eqref{m2v241m4mj1p}.
\end{proof}

%which reduces the study to the Gaussian case. 
The use of \( \mu = \mux \) from \eqref{1v2sxm12m1m} in \eqref{wBmu2vA241mmutrB} yields 
similarly to the proof of Theorem~\ref{TexpbLGA}
\begin{EQA}
	\P\Bigl( \langle \BB \xiv, \xiv \rangle > \zq^{2}(\BB,\xx), \,
		\| \HPc \BB \xiv \| \leq \zz(\mux)
	 \Bigr)
	 & \leq &
	 2 \ex^{-\xx} .
\label{2emxPblrHm1B}
\end{EQA}
%
It remains to consider the probability of large deviation
\( \P\bigl( \| \HPc \BB \xiv \| > \zz(\mux) \bigr) \).

\begin{lemma}
\label{Ldvbetagmb}
For any \( \xxc > 0 \) such that \( \zq(\BB,\xxc) + 1 \leq \gmc/\muc \), 
it holds with \( \muc = \bigl\{ 1 + \vA/(2\sqrt{\xxc}) \bigr\}^{-1} \) 
and \( \zzc = \zz(\muc) = \gmb/\muc - \sqrt{\dimA_{\HPc}/\muc} \)
\begin{EQA}
	\P\bigl( \| \HPc \BB \xiv \| > \zzc \bigr) 
	& \leq &
	\P\bigl( \langle \BB \xiv, \xiv \rangle > \zzc^{2} \bigr)
	\leq 
	\ex^{-\xxc} .
\label{exmxxlPHm1Bxigm}
\end{EQA}
\end{lemma}

\begin{proof}
It follows due to \eqref{1v2sxm12m1m} and \eqref{m2vA241muz2} for any \( \mu \leq \muc \)
\begin{EQA}
	\frac{\mu^{2} \vA^{2}}{4 (1 - \mu)} + \frac{\mu \, \dimA}{2}
	\leq 
	\frac{\muc^{2} \, \vA^{2}}{4 (1 - \muc)} + \frac{\muc \, \dimA}{2}
	& \leq &
	\frac{\muc \zq^{2}(\BB,\xxc)}{2} - \xxc ,
\label{mumucmuz2Bxmx24}
\end{EQA}
where the right hand-side does not depend on \( \mu \).
We now define \( \eta^{2} = \langle \BB \xiv, \xiv \rangle \) and use that 
\( \| \HPc \BB \xiv \| \leq \| \BB^{1/2} \xiv \| = \eta \).
Then by \eqref{wBmu2vA241mmutrB}
\begin{EQA}
	\E \exp(\mu \eta^{2}/2) \Ind\bigl( \eta \leq \zz(\mu) \bigr)
	& \leq &
	\exp \bigl\{ \muc \zq^{2}(\BB,\xxc)/2 - \xxc \bigr\} ,
\label{me22Iezmemcz2}
\end{EQA}
Define the inverse function \( \mu(\zz) = \zz^{-1}(\mu) \).
For any \( \zz \geq \zzc \), it follows from \eqref{me22Iezmemcz2} with 
\( \mu = \mu(\zz) \)
\begin{EQA}
	\E \exp\bigl\{ \mu(\zz) (\zz-1)^{2} /2 \bigr\} 
		\Ind\bigl( \zz - 1 \leq \eta \leq \zz \bigr)
	& \leq &
	\exp \bigl\{ \muc \zq^{2}(\BB,\xxc)/2 - \xxc \bigr\} 
\label{emcz2NBxm2m1I}
\end{EQA}
yielding
\begin{EQA}
	\P\bigl( \zz - 1 \leq \eta \leq \zz \bigr)
	& \leq &
	\exp \Bigl( 
		- \mu(\zz) \, (\zz - 1)^{2}/2 + \muc \zq^{2}(\BB,\xxc)/2 - \xxc  
	\Bigr)
\label{mzm12mcz2Bxm2x}
\end{EQA}
and hence,
\begin{EQA}
	\P\bigl( \eta > \zz \bigr)
	& \leq &
	\int_{\zz}^{\infty} \exp\bigl\{ - \mu(\zq) (\zq-1)^{2}/2 + \muc \zq^{2}(\BB,\xxc)/2 - \xxc \bigr\}
		d\zq
\label{zzzzcm1Pezmcl22}
\end{EQA}
Further, \( \mu \, \zz(\mu) = \gmb - \sqrt{\dimA_{\HPc} \mu} \) and
\begin{EQA}
	\gmc
	=
	\muc \, \zzc
	& \leq &
	\mu \, \zz(\mu)
	\leq 
	\gmb,
	\quad
	\mu \leq \muc .
\label{muxzxmzmglex}
\end{EQA}
This implies the same bound for the inverse function:
\begin{EQA}
	\gmc
	& \leq &
	\zz \, \mu(\zz)
	\leq 
	\gmb,
	\quad
	\zz \geq \zzc \, ,
\label{muxzxmzmglexi}
\end{EQA}
and 
\begin{EQA}
	\P\bigl( \eta > \zz \bigr)
	& \leq &
	\int_{\zz}^{\infty} 
		\exp\bigl\{ - \mu(\zq) \bigl( \zq^{2}/2 - \zq \bigr) + \muc \zq^{2}(\BB,\xxc)/2 - \xxc \bigr\} d\zq
	\\
	& \leq &
	\int_{\zz}^{\infty} 
		\exp\bigl\{ - \gmc \, \zq/2 + \gmb + \muc \, \zq^{2}(\BB,\xxc)/2 - \xxc \bigr\} d\zq
	\\
	& \leq &
	\frac{2}{\gmc}
		\exp\bigl\{ - \gmc \, \zz / 2 + \gmb + \muc \, \zq^{2}(\BB,\xxc)/2 - \xxc \bigr\} .
\label{Perzxinzinmmuz2gmz2}
\end{EQA}
Conditions \( \gmc \zzc = \muc^{-1} \gmc^{2} \geq \muc \bigl\{ \zq(\BB,\xxc) + 1 \bigr\}^{2} \)
%\( \muc \zzc = \gmc \geq \zq(\BB,\xxc) + 1 \) 
and \( \gmc \geq 1 \) 
ensure that
\( \P\bigl( \eta > \zzc \bigr) \leq \ex^{-\xxc} \).
%
\end{proof}

Remind that \( \xxc \) is the largest \( \xx \)-value ensuring the condition
\( \gmc \geq \zq(\BB,\xx) + 1 \).
We also use that for \( \xx \leq \xxc \), it holds \( \zzx = \zz(\mux) \geq \zz(\muc) = \zzc \).
Therefore, by \eqref{2emxPblrHm1B} and Lemma~\ref{Ldvbetagmb} 
\begin{EQA}
	\P\bigl( \langle \BB \xiv, \xiv \rangle \geq \zq^{2}(\BB,\xx) \bigr)
	& \leq &
	\P\bigl( \langle \BB \xiv, \xiv \rangle \geq \zq^{2}(\BB,\xx), \| \HPc \BB \xiv \| \leq \zzx \bigr)
	+ \P\bigl( \langle \BB \xiv, \xiv \rangle \geq \zzc^{2} \bigr)
	\\
	& \leq &
	2 \ex^{-\xx} + \ex^{-\xxc} \, .
\label{2emxpemxcPBxx}
\end{EQA}
Finally we consider \( \xx > \xxc \).
Applying \eqref{Perzxinzinmmuz2gmz2} yields by \( \zz \geq \zzc \)
\begin{EQA}
	\P\bigl( \eta > \zz \bigr)
	& \leq &
	\frac{2}{\muc \, \zzc}
		\exp\bigl\{ - \muc \, \zzc^{2} / 2 + \gmb + \muc \, \zq^{2}(\BB,\xxc)/2 - \xxc \bigr\}
		\exp\bigl\{ - \muc \, \zzc (\zz - \zzc) / 2  \bigr\}
	\\
	& \leq &
	\ex^{- \xxc} \exp\bigl\{ - \gmc (\zz - \zzc) / 2  \bigr\}
\label{emxcmcmzczzc2}
\end{EQA}
The choice \( \zz \) by 
\begin{EQA}
	\gmc (\zz - \zzc) / 2 
	&=&
	\xx - \xxc
\label{mzzc2xxczz}
\end{EQA}
ensures the desired bound.



%
%Define \( \Uv = \gammav/\| \gammav \| \). 
%It is easy to see that the value \( \Eg \exp\bigl( \langle \Uv,\vv \rangle \bigr) \)
%only depends on \( \zz = \| \vv \| \).
%Let us fix some \( \rr \leq \gmb \) and define
%\begin{EQA}
%	f_{\rr}(\zz) 
%	& \eqdef &
%	\Eg \exp\bigl( \rr \langle \Uv,\vv \rangle \bigr) ,
%	\qquad
%	\| \vv \| = \zz.
%\label{?}
%\end{EQA}
%Obviously \( f_{\rr}(\zz) \) is a convex function.
%Moreover, with \( \DP = \BB^{1/2} \leq \HPi \), by \eqref{expgamgm}
%\begin{EQA}
%	\E f_{\rr} \bigl( \| \DP \xiv \| \bigr)
%	&=&
%	\Eg \E_{\xiv} \exp\bigl( \rr \langle \Uv, \DP \xiv \rangle \bigr)
%	\leq 
%	\E \exp\bigl( \rr^{2} \langle \BB \Uv, \Uv \rangle / 2 \bigr) .
%\label{?}
%\end{EQA}
%By the Chebyshev inequality 
%\begin{EQA}
%	\log \P\bigl( \langle \BB \xiv, \xiv \rangle > \zq^{2} \bigr)
%	& \leq &
%	\log \E f_{\rr} \bigl( \| \DP \xiv \| \bigr) - \log f_{\rr} \bigl( \zq \bigr) 
%	\\
%	& \leq &
%	\E \exp\bigl( \rr^{2} \langle \BB \Uv, \Uv \rangle / 2 \bigr) - \log f_{\rr} \bigl( \zq \bigr)
%\label{?}
%\end{EQA}
%which again reduces the study to the Gaussian case. 
\end{proof}



==> BvM_Gauss.tex <==
% !TEX root = ../gpp_linear.tex
%\def\penm{c}

%%%%%%%%%%%%%%%%%%%%%%%%%%%   non-parametric BvM   %%%%%%%%%%%%%%%%%%%%%%
\section{Prior impact and Bayes confidence sets: Gaussian case}
\label{SPriorGauss}
  This section discusses the crucial question of the prior impact in the case of linear Gaussian model and a Gaussian prior.
  More precisely, given a Gaussian prior \(\ND(0,\GP^{-2})\), consider the corresponding 
  credible set for the posterior defined as the level set of the posterior density 
  and it is of elliptic shape.
  The first question to address is whether a credible set constructed for one prior remains 
  a nearly credible set for another one. 
  The other question is within the frequentist Bayes approach.
  Suppose that the data come from some underlying Gaussian distribution 
  with the ``true'' mean \(\thetavs\). 
  We are interested to check whether the credible set can be used as a ``honest''
  confidence set for the true mean \(\thetavs\).
  We present two different ways of looking at this problem.
  One is very strict and based on the total variation distance between the posterior and 
  the standard normal distribution.
  Such results are usually referred to as Bernstein -- von Mises Theorem.
  The second way only focuses on the elliptic sets in the parameter space.
  It turns out that the results can be drastically improved compared to the total variation approach.

  Consider a linear Gaussian model \(\Yv = \Psi^{\T} \thetavs + \sigma \epsv\) 
  with a standard Gaussian error \(\epsv \sim \ND(0,\Id_{n})\) and with a vector 
  \(\thetavs \in \R^{\infty}\) and a linear design operator 
  \(\Psi \colon \R^{\infty} \to \R^{n}\) and its adjoint \( \Psi^{\T} \).
  Define the self-adjoint operator \(\IF\) in \(\R^{\infty}\) 
  and its self-adjoint square root \(\DPc\) as
  \begin{EQA}
  	\IF 
  	& \eqdef &
  	\sigma^{-2} \Psi \Psi^{\T} ,
  	\qquad
  	\DPc^{2} = \IF .
  \label{IFPsPsTBvMi}
  \end{EQA}
  %
  Let \(\subI_{\Psi} = \Image(\Psi)\) be the subspace in \(\R^{\infty}\) spanned by the columns of 
  \(\Psi\) and let \(\Proj_{\Psi} \eqdef \Psi^{\T} (\Psi \Psi^{\T})^{-1} \Psi\) be the projector on 
  \(\subI_{\Psi}\).
  Here and in the definition of the MLE \(\tilde{\thetav} = (\Psi \Psi^{\T})^{-1} \Psi \Yv\) 
  the inversion should be understood as pseudo-inversion within \(\subI_{\Psi}\).
  %
  We suppose that the parameter space \(\Theta\) coincides with the space \(\R^{\infty}\).
  The study easily extends to the case when \(\Theta \subset \R^{\infty}\).
  Given a Gaussian prior \(\ND(0,\GP^{-2})\) with a compact operator \(\GP^{-2}\), 
  the posterior \(\vthetav_{\GP}\) is also normal, centered at 
  \(\tilde{\thetav}_{\GP} = \sigma^{-2} (\IF + \GP^{2})^{-1} \Psi \Yv\), and
  \begin{EQA}
    \bigl( \vthetav_{\GP} - \tilde{\thetav}_{\GP} \bigr) \cond \Yv
    & \sim &
    \ND(0,\DPGP^{-2}) ,
    \label{IF12vtttGPND}
    \\
    \DPGP^{2}
    & \eqdef &
    \DPc^{2} + \GP^{2} \, .
  \end{EQA}
    %
  That is, \(\vthetav_{\GP}\) given \(\Yv\) is normal vector in \(\R^{\infty}\) with mean 
  \(\tilde{\thetav}_{\GP}\) and the covariance operator \(\DPGP^{-2}\).
  One can see that the mean and the variance of the posterior \(\vthetav_{\GP}\) 
  are affected by the prior covariance \(\GP^{-2}\). 
  %
  The questions to answer are: how sensitive such credible sets are 
  to the choice of the prior covariance operator \(\GP^{2}\)?
  Can one use such credible sets as confidence sets for the true parameter \(\thetavs\)?

\subsection{Concentration sets for the posterior}
  In a linear Gaussian model and a Gaussian prior, the centered and rescaled posterior 
  \(\DPGP \bigl(\vthetav_{\GP} - \tilde{\thetav}_{\GP}\bigr)\) given \(\Yv\) 
  is a standard Gaussian measure in the Hilbert space \(\R^{\infty}\).
  Unfortunately, this measure does not concentrate on a ball of any fixed radius \(\rr\).
  %Equivalently, \(\vthetav_{\GP} \cond \Yv\) does not concentrate
  %on the ball 
  %\(\bigl\{ \thetav \colon 
  %\bigl\| \DPGP \bigl( \thetav - \tilde{\thetav}_{\GP} \bigr) \bigr\| \bigr\} \leq \rr\).
  An important question is to describe the ``smallest'' subset in \(\R^{\infty}\) on which the posterior concentrates with a large probability.
  The Gaussian structure helps to easily answer this question.
  %
  For any linear operator \(\QP\) from \(\R^{\infty}\) to \( \R^{\mm} \), the distribution of 
  \(\QP \bigl( \vthetav_{\GP} - \tilde{\thetav}_{\GP} \bigr)\) given \(\Yv\) in normal zero mean 
  with variance \(\BBQG = \QP \DPGP^{-2} \QP^{\T}\).
  %  By \(\BBQG^{1/2}\) we denote its symmetric square root.  
  %
  %  Suppose that \(\VP_{\GP}^{2}\) is invertible, 
  Typical examples of \(\QP\) are identity operator or a projector in \(\R^{\infty}\) 
  onto a finite dimensional subspace.
  Elliptic level sets of the posterior \(\QP \vthetav_{\GP}\) can be naturally used as credible sets.
  %
  Consider the rescaled posterior 
  \(\QP (\vthetav_{\GP} - \tilde{\thetav}_{\GP}) \cond \Yv\).
  It is conditionally on \(\Yv\) normal zero mean with the covariance matrix 
  \(\BBQG = \QP \DPGP^{-2} \QP^{\T}\).
  Suppose that \(\BBQG\) is a trace operator with 
  \begin{EQA}
    	\dimQG
    	& \eqdef &
    	\tr\bigl( \BBQG \bigr)
    	<
    	\infty,
  	\quad
	\varA_{\QPGP}^{2}
	\eqdef
	\tr\bigl( \BBQG^{2} \bigr),
	\quad
  	\lambda_{\QPGP} 
  	\eqdef 
  	\lambda_{\max}(\BBQG)
  	< \infty \, .
  \label{trQP2DG2i}
  \end{EQA}
  %
  Theorem~\ref{TexpbLGA} from Appendix implies that the posterior 
  \(\QP (\vthetav_{\GP} - \tilde{\thetav}_{\GP}) \cond \Yv = \ND(0, \BBQG)\) 
  concentrates with probability at least \(1 - \ex^{-\xx}\) on the set 
  \(\bigl\{ \thetav \colon \bigl\| \QP \bigl( \thetav - \tilde{\thetav}_{\GP} \bigr) \bigr\| \leq \rr \bigr\}\)
  for 
  \begin{EQA}
  	\rr
  	& \geq &
  	\zq(\BBQG, \xx) 
	\eqdef 
	\sqrt{\dimQG + 2 \varA_{\QPGP} \, \xx^{1/2} + 2 \lambda_{\QPGP} \, \xx}
	\leq 
	\sqrt{\dimQG} + \sqrt{2 \lambda_{\QPGP} \, \xx} \, .
	\qquad
  \label{rrzqdGxspG2x}
  \end{EQA}
    %
    %  In particular, with \(\QP = \DPc\), it holds 
    %  \(\DPc (\vthetav_{\GP} - \tilde{\thetav}_{\GP}) \cond \Yv \sim \ND(0,\BB)\)
    %  for \(\BB = \DPc \, \DPGP^{-2} \DPc\),
    %  and we only need \(\BP\) to be a trace operator.

  \begin{theorem}
  \label{TBvMgausscont}
  Let a linear operator \(\QP\) be such that \(\BBQG = \QP \DPGP^{-2} \QP^{\T}\) satisfies \eqref{trQP2DG2i}.
  %
  Then for any \(\xx \geq 0\), it holds almost surely with 
  \(\zq(\BBQG, \xx)\) from \eqref{rrzqdGxspG2x}
  \begin{EQA}
    	\P\Bigl( 
      	\bigl\| \QP \bigl( \vthetav_{\GP} - \tilde{\thetav}_{\GP} \bigr) \bigr\| 
      	\geq \zq(\BBQG, \xx) \cond \Yv 
    	\Bigr)
    	& \leq &
    	\ex^{-\xx} \, .
  \label{PQvtGttGzqx}
  \end{EQA} 
  \end{theorem}
  

\subsection{Nonparametric BvM Theorem: Gaussian case}
\label{SBvMGauss}
  This section discusses a version of the BvM result which compares the posterior distribution \(\ND(\tilde{\thetav}_{\GP},\BBQG)\) of 
  \(\QP \vthetav_{\GP}\) given \(\Yv\) with the normal distribution \(\ND(\thetavs, \BB_{\QP})\) 
  which is the distribution of \(\QP \tilde{\thetav}\).
  Here \(\BB_{\QP} = \QP \DPc^{-2} \QP^{\T}\), it coincides with \(\BBQG\) for \(\GP^{2} = 0\). 
  Equivalently, we compare two different posteriors, one for the prior \(\ND(0,\GP^{-2})\), 
  and the other one, for the improper non-informative prior with \(\GP^{2} = 0\).
  The standard issue for this comparison is to quantify the change of the mean and variance 
  in the posterior distribution induced by the Gaussian prior. 
  However, in the nonparametric framework, there is an additional problem because 
  a Gaussian measure in the infinite dimensional space is only defined in a weak sense 
  while the BvM result is oriented towards the strong total variation distance.

  To simplify the presentation, assume that \(\QP\) maps \(\R^{\infty}\) onto 
  a finite dimensional space \(\R^{\mm}\) and the operator 
  \(\BBQG = \QP \DPGP^{-2} \QP^{\T}\) in \(\R^{\mm}\) is invertible.
  %  Also define \(\BB = \QP \DPc^{-2} \QP^{\T}\) which corresponds to \(\GP = 0\).
  For two Gaussian measures in \(\R^{\infty}\), 
  the total variation distance between them 
  can be upper bounded using the Pinsker inequality; see Lemma~\ref{KullbTVd} in the Appendix.
  Namely, define two quantities 
  \(\errSi_{\QPGP}\) and \(\bias_{\QPGP}\) 
  \begin{EQA}
  \label{trQPPrG}
    \errSi_{\QPGP}^{2}
    & \eqdef &
    \tr \bigl\{ (\BBQG^{-1/2} \BB_{\QP} \BBQG^{-1/2} - \Id)^{2} \bigr\} ,
    \\
    % \bias_{\QPGP}^{2}
    % & \eqdef &
    % \bigl( \tilde{\thetav}_{\GP} - \tilde{\thetav} \bigr)^{\T} \VP_{\GP}^{-2} \VP^{2} \VP_{\GP}^{-2} 
    % \bigl( \tilde{\thetav}_{\GP} - \tilde{\thetav} \bigr) .  
    \bias_{\QPGP}
    & \eqdef &
    %    \bigl( \tilde{\thetav}_{\GP} - \tilde{\thetav} \bigr)^{\T} 
    \bigl\| \BB_{\QP}^{1/2} \BBQG^{-1} \bigl( \tilde{\thetav}_{\GP} - \tilde{\thetav} \bigr) \bigr\|.  
  \label{PrGQPt}
  \end{EQA}
  %
  Although a BvM type statement does not hold on the entire space \(\R^{\infty}\), 
  the next result claims that it is nearly true after mapping 
  \(\QP \colon \R^{\infty} \to \R^{\mm}\) 
  under the constraint ``\(\errSi_{\QPGP}\) and \(\bias_{\QPGP}\) are small''.

  \begin{theorem}
  \label{TBvMlinGaussprior}
    Given \(\QP \colon \R^{\infty} \to \R^{\mm}\),
    consider the posterior distribution \(\posterior_{\QPGP}\) of \(\QP \vthetav_{\GP}\) given \(\Yv\) for a linear Gaussian model 
    \(\Yv = \Psi^{\T} \thetav + \sigma \epsv\) with a standard Gaussian error 
    \(\epsv \sim \ND(0,\Id_{n})\) for a Gaussian prior \(\ND(0,\GP^{-2})\).
    Define %\(\RR = \DPc^{-1} \GP^{2} \DPc^{-1}\)
    \begin{EQ}[lcl]
    	\DPc^{2} 
    	& = &
    	\sigma^{-2} \Psi \Psi^{\T} ,
    	\\
    	\DPGP^{2}
    	& = &
    	\sigma^{-2} \Psi \Psi^{\T} + \GP^{2} \, ,
    	\\
    	\tilde{\thetav} 
    	&=& 
    	\bigl( \Psi \Psi^{\T} \bigr)^{-1} \, \Psi \, \Yv \, ,
    	\\
    	\tilde{\thetav}_{\GP}
    	&=& 
    	\bigl( \Psi \Psi^{\T} + \sigma^{2} \GP^{2} \bigr)^{-1} \, \Psi \, \Yv 
	=
	\sigma^{-2} \DPGP^{-2} \Psi \Yv
	\, .
    \label{IFGPdefBvMig}
    \end{EQ}
    %
    Let \(\posterior_{\QP}\) correspond to 
    \(\GP = 0\), \(\posterior_{\QP} = \ND(\QP \tilde{\thetav}, \QP \DPc^{-2} \QP^{\T})\).
    Let the values \(\errSi_{\QPGP}\) and \(\bias_{\QPGP}\) be given by \eqref{trQPPrG} 
    and \eqref{PrGQPt}. 
    %  Let \(\B(\subI)\) be a collection of all Borel sets on \(\subI\).
    Then it holds 
    \begin{EQA}
    	\| \posterior_{\QPGP} - \posterior_{\QP} \|_{\TV}
    	& \eqdef &
    	\sup_{A \in \B(\R^{\mm})}
    	\bigl| 
      	\P \bigl\{ 
        		\QP \bigl( \vthetav_{\GP} - \tilde{\thetav} \bigr) \in A \cond \Yv
      	\bigr\}
      	- \P\bigl(\QP \DPc^{-1} \gaussv \in A\bigr) 
    	\bigr|
    	\\
    	& \leq &
    	\frac{1}{2} \sqrt{\errSi_{\QPGP}^{2} + \bias_{\QPGP}^{2}}
    \label{supABIPcPg}
    \end{EQA}
    for a standard Gaussian vector \(\gammav\) in \(\R^{\mm}\).
  \end{theorem}

  \noindent
  Below we consider a couple of examples met in the literature.
  First we analyze the variance term \(\errSi_{\QPGP}\).

  \begin{example}
  \label{ExsIFnIng}
    Let 
    \(\sigma^{2} = 1\), \(\IF = \IF_{n} = n \Id_{n}\), 
    and let \( \gp_{1}^{2} \leq \gp_{2}^{2} \leq \ldots \) be a growing sequence satisfying 
    \( \sum_{j} \gp_{j}^{-2} < \infty \).
    Define \( \NE \) as the smallest index \( j \) under the relation \( \gp_{\NE}^{2} \geq \nsize \).
    Now define the penalization matrix as
    \(\GP^{2} = \diag\{ 0,\ldots,0, \gp_{\NE}^{2}, \gp_{\NE+1}^{2},  \ldots \}\).
    Then \(\DPc^{2} = n \Id_{n}\),
    \(\DPGP^{2} = n \Id_{n} + \GP^{2} \).
    This is a diagonal matrix as well with the diagonal entries \( n + \gp_{j}^{2} \Ind(j \geq \NE) \).
    Let also \(\QP = \nsize^{1/2} \Proj_{\mm}\) for some index \( \mm \). 
%   Now for a fixed \(\mm\), consider the subspace \(\subI_{\mm}\) spanned by the first \(\mm\) basis elements.
%    For \(j \leq \mm\), it holds
%    \begin{EQA}
%    	1 - \frac{1}{1 + \gp_{j}^{2}/n}
%    	& = &
%    	\frac{\gp_{j}^{2}/n}{1 + \gp_{j}^{2}/n}
%    	\leq 
%    	\frac{\gp_{\mm}^{2}/n}{1 + \gp_{\mm}^{2}/n}.
%    \label{1fr11gpj2n}
%    \end{EQA}
    %
%    The value \(\errSi_{\QPGP}\) can be bounded as follows.
	If \( \mm < \NE \), then the effect of penalization in the product \( \QP \vthetav_{\GP} \) disappears, 
	and \( \errSi_{\QPGP} = 0 \), \( \bias_{\QPGP} = 0 \).
    If \( \mm \geq \NE \), then
    \begin{EQA}
    	\errSi_{\QPGP}^{2}
    	&=&
    	\sum_{j=\NE}^{\mm} \biggl(1 - \frac{1}{1 + \gp_{j}^{2}/n} \biggr)^{2}
    	=
    	\sum_{j=\NE}^{\mm} \frac{\gp_{j}^{4}/n^{2}}{(1 + \gp_{j}^{2}/n)^{2}}
    	\leq 
		\mm - \NE + 1 .
%    	\frac{L^{2}}{4 \beta + 1} n^{-2} \NE^{4 \beta + 1}.
    \label{errSibetap1}
    \end{EQA}
    Similar arguments imply
    \begin{EQA}
    	\errSi_{\QPGP}^{2}
    	& \geq &
		\frac{\mm - \NE + 1}{4} \, .
%    	\frac{L^{2}}{4 \beta + 1} n^{-2} \NE^{4 \beta + 1}.
    \label{errSibetap1}
    \end{EQA}
    %
One can conclude that the Pinsker inequality fails to show BvM type results if 
\( \mm \geq \NE \). 
%For the opposite case \( \mm < \NE \), 
%\begin{EQA}
%	\errSi_{\QPGP}^{2}
%    & \asymp &
%	\frac{1}{\nsize^{2}}\sum_{j=1}^{\mm} \gp_{j}^{4} \, .
%\label{errQG21n2s1jm4}
%\end{EQA}
%In particular, in the roughness penalty approach, \(\gp_{j}^{2} = L j^{2\beta}\) for \(\beta > 0\).
%Then 
%\( \sum_{j=1}^{\mm} \gp_{j}^{4} \approx \frac{L^{2}}{4 \beta + 1} n^{-2} \mm^{4 \beta + 1} \),
%and the condition ``\( \errSi_{\QPGP} \) is small'' reads as \( L^{2} \mm^{4 \beta + 1} \ll \nsize^{2} \).
  \end{example}

Now we compare two different diagonal priors with covariance operators \( \GP^{-2} \neq \GP_{1}^{-2} \) yielding two 
different Gaussian posteriors \(\posterior_{\QPGP} = \ND(\QP \tilde{\thetav}_{\GP}, \QP \DPGP^{-2} \QP^{\T})\) and \(\posterior_{\QPGP_{1}} = \ND(\QP \tilde{\thetav}_{\GP_{1}}, \QP \DP_{\GP_{1}}^{-2} \QP^{\T})\).

  \begin{example}
  \label{LexamGPP}
    Let as in previous example, \(\IF = \nsize \Id_{\nsize} \) and \( \QP = \nsize^{1/2} \Proj_{\mm} \).
    For two given growing sequences \( \bigl( \gp_{j}^{2} \bigr) \) and \( \bigl( \gp_{j,1}^{2} \bigr) \) with 
    \( \gp_{j,1}^{2} \leq \gp_{j}^{2} \), let the values \( \NE \) and \( \NE_{1} \) and the matrices 
    \( \GP^{2} \) and \( \GP_{1}^{2} \) be defined as in Example~\ref{ExsIFnIng}.
    Obviously \( \NE_{1} \geq \NE \).
    If \( \mm < \NE \), then \( \QP \vthetav_{\GP} \) and \( \QP \vthetav_{\GP_{1}} \) coincide.
    If \( \NE_{1} > \NE \) and \( \mm \geq \NE \), then similarly to Example~\ref{ExsIFnIng}
\begin{EQA}
	\errSi_{\QP}^{2}\bigl( \GP,\GP_{1} \bigr)
    & \eqdef &
    \tr \bigl\{ (\BBQG^{-1/2} \BB_{\QPGP_{1}} \BBQG^{-1/2} - \Id)^{2} \bigr\}
    \geq 
    \frac{\mm - \NE + 1}{4} .
\label{dn2G1GDG1G}
\end{EQA}
    Finally, if \( \NE = \NE_{1} \) and \( \mm \geq \NE \), define
\begin{EQA}
	\delta_{\mm}(\GP,\GP_{1})
	& \eqdef &
	\max_{\NE \leq j \leq \mm} \frac{\gp_{j}^{2} - \gp_{j,1}^{2}}{\nsize + \gp_{j,1}^{2}} \, .
\label{dmG1Gnj1mgj2}
\end{EQA}
Then \( \errSi_{\QP}\bigl( \GP_{1},\GP \bigr) \geq \delta_{\mm}(\GP_{1},\GP) \), and
therefore, it suffices to have one component \( j \in [\NE,\mm] \), for which 
\( (\gp_{j}^{2} - \gp_{j,1}^{2}) / \gp_{j,1}^{2} \) is significantly positive to indicate
a significant difference between the posteriors \( \posterior_{\QPGP} \) and \( \posterior_{\QPGP_{1}} \).
  \end{example}


%    Now we consider a slightly different situation when the prior covariance operator 
%    \(\GP^{2} = \tau_{n}^{2} \Proj_{\subI}\) coincides up to a constant factor with the projector 
%    \(\Proj_{0}\) on the subspace \(\subI\) of dimension \(\mm = \dimn\) spanned by the 
%    first basis eigenvectors.
%    Then \(\DPGP^{2} = \sigma_{n}^{2} \Id + \tau_{n}^{2} \Id_{\subI}\) and 
%    \(\Projs_{\GP} = \bigl( \Id + (\tau_{n}/\sigma_{n})^{2} \Id_{\subI} \bigr)^{-1}\).
%    Therefore,
%    \begin{EQA}
%    	\errSi_{\QPGP}^{2}
%    	&=&
%    	\sum_{j=1}^{\dimn} \biggl( 1 - \frac{1}{1 + (\tau_{n}/\sigma_{n})^{2}} \biggr)^{2}
%    	\leq 
%    	\dimn (\tau_{n}/\sigma_{n})^{4} .
%    \label{errSibetaptaun}
%    \end{EQA}
%    %
%    This leads to the condition on the dimensionality \(\dimn\) of \(\subI\): \(\dimn (\tau_{n}/\sigma_{n})^{4} \to 0\) as \(n \to \infty\)  which coincides with~\cite{Bo2011} and~\cite{Jo2012}.


\subsection{Credible sets and Gaussian comparison}
\label{SCSGaussComp}
  This section revisits the problem of prior impact.
  The only difference between the results from Section~\ref{SBvMGauss} and from this section is that we focus now on the credible sets with elliptic shape.
  % which are the level sets of the posterior density. 
  Remind that the Gaussian prior \(\ND(0,\GP^{-2})\) in the linear Gaussian model leads to the Gaussian posterior \(\ND\bigl( \tilde{\thetav}_{\GP}, \DPGP^{-2} \bigr)\).
  For a linear operator \(\QP\), the random element \(\QP \, \vthetav_{\GP}\) is conditionally on 
  \(\Yv\) normal with mean \(\QP \, \tilde{\thetav}_{\GP}\) and the covariance 
  \(\BBQG = \QP \DPGP^{-2} \QP^{\T}\).
  A natural construction of the credible sets for this posterior is given by 
  \begin{EQA}
  	\CS_{\QPGP}(\rr)
  	& \eqdef &
  	\Bigl\{ \thetav \colon 
  		\bigl\| \QP \bigl( \thetav - \tilde{\thetav}_{\GP} \bigr) \bigr\| \leq \rr
  	\Bigr\}.
  \label{CSrrtcDGtttG}
  \end{EQA}
    %
  Given \(\alp\), one can fix the radius \(\rr_{\QPGP}\) to ensure the posterior probability 
  \(1 - \alp\) for the set \(\CS_{\GP}(\rr_{\QPGP})\). 
  The question of a prior impact can be stated as follows: 
  whether the obtained credible sets significantly depend on the prior covariance \(\GP^{-2}\). 
  Consider another prior \( \ND(0, \GP_{1}^{-2})\) with the covariance operator 
  \(\GP_{1}^{-2}\).
  The non-informative improper prior formally corresponds to \(\GP_{1}^{2} = 0\).
  The posterior \(\vthetav_{\GP_{1}}\) is again normal but now with parameters 
  \(\tilde{\thetav}_{\GP_{1}} = \bigl( \Psi \Psi^{\T} + \sigma^{2} \GP_{1}^{2} \bigr)^{-2} \Psi \Yv\) 
  and \(\DP_{\GP_{1}}^{2} = \sigma^{-2} \Psi \Psi^{\T} + \GP_{1}^{2}\).
  We aim at checking the \(\GP_{1}\)-posterior probability of the credible set 
  \(\CS_{\QPGP}(\rr_{\QPGP})\):
  \begin{EQA}
  	\P\bigl(\vthetav_{\GP_{1}} \not\in \CS_{\QPGP}(\rr_{\QPGP}) \cond \Yv \bigr)
  	&=&
  	\P\Bigl( 
  		\bigl\| \QP \bigl( \vthetav_{\GP_{1}} - \tilde{\thetav}_{\GP} \bigr) \bigr\| 
  		\geq \rr_{\QPGP} \cond \Yv 
  	\Bigr).
  \label{PG1QvttGrG}
  \end{EQA}
  Results of this paper allow to significantly improve the bound of the previous section based on the Pinsker inequality and the Kullback-Leibler distance between two Gaussian posteriors. 
  In particular, only the nuclear (Schatten-one) norm \(\bigl\|\BBQG - \BB_{\QPGP_{1}}\bigr\|_{1}\), the norm of the vector \(\av\), and
  the Frobenius norm of \(\BBQG\) are involved in the new bounds.
  The only technical condition concerns the first three eigenvalues of \(\BBQG\).
  Effectively it requires that \( \QP \) is at least three dimensional.
  In particular, the result does not apply to linear functional of \( \thetav \).
  We state the result in a simplified form, further options can be found 
  in Section~\ref{SGausscomp}.

  \begin{theorem}
  \label{TBvMGauss}
    Let Gaussian priors \( \ND(0, \GP^{-2})\) and 
    \( \ND(0, \GP_{1}^{-2})\) be fixed. % and \( \GP^{2} \geq \GP_{1}^{2} \).
    Let also \(\QP^{\T} \QP \leq \DPGP^{2}\) 
    %
    and \(\BBQG = \QP \DPGP^{-2} \QP^{\T}\) satisfy \(\tr \BBQG \geq 3\),
    and similarly, \(\QP^{\T} \QP \leq \DP_{\GP_{1}}^{2}\), 
    \(\tr\BB_{\QPGP_{1}} \geq 3\).
    Let, given \(\alp\), the credible set \(\CS_{\QPGP}(\rr_{\QPGP})\) have the posterior probability
    \(1 - \alp\) for the prior measure \( \ND(0,\GP^{-2})\).
    Then it holds  
    \begin{EQA}
    	&& \nquad
		\bigl|\P\bigl( \vthetav_{\GP_{1}} \not\in \CS_{\QPGP}(\rr_{\QPGP}) \cond \Yv \bigr)
    	- \alp \bigr|
    	\\
		& \lesssim &
    	\biggl(
    		\frac{1}{\| \BBQG \|_{\Fr}} 
    		+ \frac{1}{\| \BB_{\QPGP_{1}} \|_{\Fr}}
    		\biggr) 
    		\biggl( \bigl\| \BBQG - \BB_{\QPGP_{1}} \bigr\|_{1} 
			+ \bigl\| \QP\bigl( \tilde{\thetav}_{\GP} - \tilde{\thetav}_{\GP_{1}} \bigr)\bigr\|^{2}\biggr) .
    \label{tv_main_bound}
    \end{EQA}
%    with 
%    \begin{EQA}
%    	\av
%    	& \eqdef &
%    	\QP\bigl( \tilde{\thetav}_{\GP} - \tilde{\thetav}_{\GP_{1}} \bigr).
%    \label{aWtGtG1def}
%    \end{EQA}
  \end{theorem}


  \begin{proof}
%    .
    The calibration condition for the credible set \(\CS_{\QPGP}(\rr_{\QPGP})\)
    can be written as 
\begin{EQA}
	\P\bigl( \| \QP (\vthetav_{\GP} - \tilde{\thetav}_{\GP}) \| \geq \rr_{\QPGP} \cond \Yv \bigr) 
	&=& 
	\alp.
\label{PcalQtGttGrGYa}
\end{EQA}
	We want to check the probability of the same set under the prior \(\ND(0, \GP_{1}^{-2})\):
    \begin{EQA}[c]
    	\P\Bigl( 
			\bigl\| \QP (\vthetav_{\GP_{1}} - \tilde{\thetav}_{\GP}) \bigr\| \geq \rr_{\QPGP} \cond \Yv
		\Bigr) .
    \label{PxiG1marG1}
    \end{EQA}
    Introduce \(\xiv_{\GP} \sim \ND(0, \BB_{\QPGP})\), 
    \(\xiv_{\GP_{1}} \sim \ND(0, \BB_{\QPGP_{1}})\). 
    The conditional distribution of \( \QP (\vthetav_{\GP} - \tilde{\thetav}_{\GP}) \) given \(\Yv\) 
    coincides with the distribution of \( \xiv_{\QPGP} \). %zero mean Gaussian with covariance \(\BBQG\).
    Similarly \( \QP (\vthetav_{\GP_{1}} - \tilde{\thetav}_{\GP}) \cond \Yv \sim \ND(0,\BB_{\QPGP_{1}}) 
    = \LL(\xiv_{\GP_{1}})\), and
    \begin{EQA}
    %	&& \nquad
    	\left| 
    		\P\Bigl( 
    			\bigl\| \QP \bigl( \vthetav_{\GP_{1}} - \tilde{\thetav}_{\GP} \bigr) \bigr\|	
				\geq \rr_{\QPGP} \cond \Yv 
    		\Bigr) - \alpha 
    	\right|
    %	\\
    	& \leq &
    	\sup_{\rr > 0} \left| 
    		\P\Bigl( \bigl\| \xiv_{\GP_{1}} - \av \bigr\| \geq \rr \Bigr) 
    		- \P\Bigl( \bigl\| \xiv_{\GP} \bigr\| \geq \rr \Bigr)
    	\right| \, ,
    \label{PG1WvttGrGPr}
    \end{EQA}
    The result follows by Theorem~\ref{Tgaussiancomparison3} with 
    \( \av = \QP\bigl( \tilde{\thetav}_{\GP} - \tilde{\thetav}_{\GP_{1}} \bigr) \).
  \end{proof}

  \begin{remark}
    If \(\GP^{2} \geq \GP_{1}^{2}\), then \(\BB_{\QPGP} \leq \BB_{\QPGP_{1}}\) and
    \begin{EQA}
    	\bigl\|\BB_{\QPGP} - \BB_{\QPGP_{1}}\bigr\|_{1}
    	&=&
    	\tr \BB_{\QPGP_{1}} - \tr \BB_{\QPGP}
    \label{SGmSG1tGtG1}
    \end{EQA}
    and thus, the result of Theorem~\ref{Tgaussiancomparison3} 
    can be written as
    \begin{EQA}
    	\left| 
    		\P\Bigl( \bigl\| \QP \bigl( \vthetav_{\GP_{1}} - \tilde{\thetav}_{\GP} \bigr) \bigr\| 
    		\geq 
    		\rr_{\QPGP} \cond \Yv \Bigr) - \alpha 
    	\right|
    	& \leq &
    	\frac{\CONST\bigl( \tr \BB_{\QPGP_{1}} - \tr \BB_{\QPGP} 
				+ \| \QP(\tilde{\thetav}_{\GP} - \tilde{\thetav}_{\GP_{1}}) \|^{2} \bigr)}
    		 {\| \BB_{\QPGP} \|_{\Fr}} \, .
    \label{PG1QvttGrGcYC12}
    \end{EQA}
  \end{remark}

    Now we consider the bias term \(\av = \QP\bigl( \tilde{\thetav}_{\GP} - \tilde{\thetav}_{\GP_{1}} \bigr) \).
    The definition implies with \(\E \Yv = \fvs\)
    \begin{EQA}
    	\av
		=
		\QP \bigl( \tilde{\thetav}_{\GP} - \tilde{\thetav}_{\GP_{1}} \bigr)
    	&=&
    	\QP \bigl( \DPGP^{-2} - \DP_{\GP_{1}}^{-2} \bigr) \Psi \Yv
    	=
    	\QP \bigl( \DPGP^{-2} - \DP_{\GP_{1}}^{-2} \bigr) \Psi (\fvs + \epsv) .
%		+ \QP \bigl( \DPGP^{-2} - \DP_{\GP_{1}}^{-2} \bigr) \Psi \fvs
%    	\\
%    	&=&
%    	\Pi_{\subI} \bigl( \Projs_{\GP} - \Proj_{\Psi} \bigr) \DPc^{-1} \Psi \fvs 
%    	+ \Pi_{\subI} \bigl( \Projs_{\GP} - \Proj_{\Psi} \bigr) \xiv,
    \label{IF12ttGttb}
    \end{EQA}
%    where \(\xiv \eqdef \DPc^{-1} \Psi \epsv\) and 
%    \(\Cov(\xiv) = \DPc^{-1} \Psi^{\T} \Cov(\epsv) \, \Psi \, \DPc^{-1} = \Proj_{\Psi}\). 
    It holds for the stochastic part 
    \( \xiv = \QP \bigl( \DPGP^{-2} - \DP_{\GP_{1}}^{-2} \bigr) \Psi \epsv \) under \( \Var( \Psi \epsv) = \DPc^{2} \)
    \begin{EQA}
    	\E \| \xiv \|^{2}
    	&=&
    	\tr\bigl\{ \QP \bigl( \DPGP^{-2} - \DP_{\GP_{1}}^{-2} \bigr) \DPc^{2} 
			\bigl( \DPGP^{-2} - \DP_{\GP_{1}}^{-2} \bigr) \QP^{\T} \bigr\} 
    	\\
		&=&
		\tr \bigl\{ \QP \DPc^{-1} \bigl( \BB_{\GP} - \BB_{\GP_{1}} \bigr)^{2} \DPc^{-1} \QP^{\T} \bigr\} .
%		\leq 
%    	\errSi_{\QPGP}^{2} \,.
    % 	\leq 
    % 	\reps^{2} \dimre \, .
    \label{EPrGPr2de}
    \end{EQA}
    In a special case when \( \QP \DPc^{-1} \) is a projector on linear subspace of dimension \( m \),
    it holds 
\begin{EQA}
	\tr \bigl\{ \QP \DPc^{-1} \bigl( \BB_{\GP} - \BB_{\GP_{1}} \bigr)^{2} \DPc^{-1} \QP^{\T} \bigr\}
	&=&
	\tr \bigl\{ \Proj_{m} \bigl( \BB_{\GP} - \BB_{\GP_{1}} \bigr)^{2} \Proj_{m}^{\T} \bigr\}
	\\
	&=&
	\tr \bigl\{ \bigl( \BB_{\QP|\GP} - \BB_{\QP|\GP_{1}} \bigr)^{2} \bigr\}
	\leq 
	\errSi_{\QP}^{2}\bigl( \GP,\GP_{1} \bigr).
\label{trQDm1BGBG12Der}
\end{EQA}    
    %
    If \(\xiv\) is standard Gaussian one can apply the result of Theorem~\ref{TexpbLGA} to bound 
    \begin{EQA}
    	\| \xiv \|^{2}
    	& \leq & 
    	\CONST \E \| \xiv \|^{2} 
    \label{PGmIxiv}
    \end{EQA}
    on a set of dominating probability.
    In the non-Gaussian situation the value \(\| \xiv \|^{2}\) 
    can be bounded in a similar way using Theorem~\ref{LLbrevelocroB}.
    Under noise misspecification, the identity \( \Cov(\Psi \epsv) = \DPc^{2} \) does not apply
    any more. 
    However, one can obtain a similar bound for a regular noise \(\Cov (\Psi \epsv) \leq \fis^{2} \DPc^{2}\) with an additional \(\fis\) factor.  
    So, the stochastic term in \eqref{IF12ttGttb} can be controlled if \(\errSi_{\QPGP}\) is small.
%    
    The value \(\| \QP \bigl( \DPGP^{-2} - \DP_{\GP_{1}}^{-2} \bigr) \Psi \fvs \|\) can be bounded under smoothness 
    conditions on \(\fvs\); see Example~\ref{ex:rough_credible2} below.


  Now we continue the study of Example~\ref{ExsIFnIng}.
  \begin{example}[Continuation of Example~\ref{ExsIFnIng}]
  \label{ex:rough_credible}
    Given a growing sequence \( (\gp_{j}^{2}) \), 
    consider \( \NE = \min\bigl\{ j \colon \gp_{j}^{2} \geq \nsize \bigr\} \),
     \( \DPGP^{2} = \diag\bigl\{ \nsize + \gp_{j}^{2} \Ind(\gp_{j}^{2} \geq \nsize) \bigr\} \), and \( \QP = \nsize^{1/2} \Proj_{\mm} \).
     Again, for \( \mm \leq \NE \) there is no prior impact. 
    %
    Suppose that \( \gp_{j}^{2} \) grow rapidly so that \( \alp(\mm) = g_{\mm}^{2} \sum_{j \geq \mm} \gp_{j}^{-2} \) is bounded for all \( \mm \geq \NE \).
    This corresponds to a polynomial growth of \( \gp_{j} \), e.g. 
    \( \gp_{j}^{2} \approx L j^{2\beta} \) for \( \beta > 1/2 \). 
    For \( \mm > \NE \), compute
    \begin{EQA}[c]
      \|\BB_{\QPGP}\|_{\Fr}^{2} 
      =
      \tr \bigl( \QP \DPGP^{-2} \QP^{\T} \bigr)^{2}
      =
      \NE + \sum_{j=\NE}^{\mm} \biggl( \frac{n}{n + \gp_{j}^{2}} \biggr)^{2}
      \leq 
      \NE + \sum_{j=\NE}^{\mm} \frac{\gp_{\NE}^{2}}{\gp_{j}^{2}}
      =  
     \NE + \alp(\NE) \, . 
%      \sqrt{\sum_{j = 1}^{\mm} \frac{1}{(1 + \gp_{j}^{2} / \nsize)^{2}}}.
    \end{EQA}
    %
%
    Also for \( \mm \geq \NE \)
    \begin{EQA}
    	\frac{\tr \BB_{\QP} - \tr \BB_{\QPGP}}{\| \BB_{\QPGP} \|_{\Fr}}
		&=&
		\frac{1}{\| \BB_{\QPGP} \|_{\Fr}} 
			\sum_{j=\NE}^{\mm} \biggl( 1 - \frac{\nsize}{\nsize + \gp_{j}^{2}} \biggr)
		\lesssim 
		\frac{\mm - \NE}{\sqrt{\NE}}
    \end{EQA}
This value is small if \( \mm - \NE \ll \sqrt{\NE} \).
  \end{example}


  \begin{example}[Continuation of Example~\ref{LexamGPP}]
  \label{ex:rough_credible2}
  Now we compare two different posteriors for the priors from Example~\ref{LexamGPP}.
  Suppose that \( \NE_{1} > \NE \) and \( \mm \) is very large or infinite. 
  Let \( \alp_{1}(\mm) = g_{\mm,1}^{2} \sum_{j \geq \mm} \gp_{j,1}^{-2}Ê\leq \CONST \) for
  \( \mm \geq \NE_{1} \).
  Then, using \( \| \BB_{\QPGP} \|_{\Fr}^{2} \asymp \NE \),
\begin{EQA}
	\frac{\tr \BB_{\QPGP_{1}} - \tr \BB_{\QPGP}}{\| \BB_{\QPGP} \|_{\Fr}}
	&=&
	\frac{1}{\| \BB_{\QPGP} \|_{\Fr}} 
		\sum_{j=\NE}^{\NE_{1}-1} \frac{\gp_{j}^{2}}{\nsize + \gp_{j}^{2}} 
	+ \frac{1}{\| \BB_{\QPGP} \|_{\Fr}} 
	\sum_{j=\NE_{1}}^{\mm} \frac{\gp_{j}^{2} - \gp_{j,1}^{2}}{(\nsize + \gp_{j}^{2}) (\nsize + \gp_{j,1}^{2})} 
	\\
	& \lesssim &
	\frac{\NE_{1} - \NE + \alp_{1}(\NE_{1})}{\sqrt{\NE}} \, .
\label{MM1aMsMB1Fg1}
\end{EQA}  
Finally we discuss the Bayesian bias 
\( \av = \QP \bigl( \tilde{\thetav}_{\GP} - \tilde{\thetav}_{\GP_{1}} \bigr) 
= \QP \bigl( \DP_{\GP_{1}}^{-2} - \DPGP^{-2} \bigr) \Psi \Yv \).
General results for quadratic forms allow to bound 
\( \| \av \|^{2} \approx \E \| \av \|^{2} \); see Theorem~\ref{TexpbLGA}.
It holds \( \E \| \av \|^{2} =	\| \E \av \|^{2} + \tr \Var(\av) \), and 
under correct noise specification \( \Var(\Psi \epsv) = n \Id_{n} \),
\begin{EQA}
	\tr \Var(\av)
	&=&
	\nsize \tr \bigl\{ \QP \bigl( \DP_{\GP_{1}}^{-2} - \DPGP^{-2} \bigr)^{2} \QP^{\T} \bigr\}
	\\
	&=&
	\frac{1}{\nsize} \sum_{j=\NE}^{\NE_{1}-1} \frac{\gp_{j}^{4}}{(\nsize + \gp_{j}^{2})^{2}}
	+ \nsize \sum_{j=\NE_{1}}^{\mm} 
		\frac{(\gp_{j}^{2} - \gp_{j,1}^{2})^{2}}{(\nsize + \gp_{j}^{2})^{2} (\nsize + \gp_{j,1}^{2})^{2}}
	\\
	&=&
	\frac{1}{\nsize} \sum_{j=\NE}^{\NE_{1}-1} 1
	+ \sum_{j=\NE_{1}}^{\mm} \frac{1}{\nsize + \gp_{j,1}^{2}}
	\leq 
	\frac{\NE - \NE_{1} + \alp_{1}(\NE_{1})}{\nsize} \, .
\label{tVanQDGG1QT}
\end{EQA}
The squared bias \( \| \E \av \|^{2} \) can be bounded as follows:
with \( \Zv = \nsize^{-1/2} \Psi \fvs \), 
\begin{EQA}
	\| \E \av \|^{2}
	&=&
	\sum_{j=\NE}^{\NE_{1}-1} \frac{\gp_{j}^{4} z_{j}^{2}}{(\nsize + \gp_{j}^{2})^{2}}
	+ \sum_{j=\NE_{1}}^{\mm} 
		\frac{\nsize^{2} (\gp_{j}^{2} - \gp_{j,1}^{2})^{2} z_{j}^{2}}{(\nsize + \gp_{j}^{2})^{2} (\nsize + \gp_{j,1}^{2})^{2}}
	\leq
	\sum_{j=\NE}^{\mm} z_{j}^{2} \, . 
\label{gj122jMzj2}
\end{EQA}
Under standard Sobolev type smoothness conditions on \( \fvs \), 
the value \( \sum_{j=\NE}^{\mm} z_{j}^{2} \leq \| \Proj_{\NE} \fvs \|^{2} \) is small.
So, the bound \eqref{tv_main_bound} yields that
two priors with the inverse covariances \( \GP^{2} \geq \GP_{1}^{2} \) lead to nearly the same 
credible sets provided that \( \NE - \NE_{1} \ll \sqrt{\NE} \), \( \NE \) is large and that
\( \| \Pi_{\NE} \fvs \|^{2} \) is small.
  \end{example}

\subsection{Hierarchical priors}
\label{Scompprior}
The aim of this section is to understand the behavior of the hyperposterior 
\( \hyper \cond \Yv \) for a given hyperprior \( \priorh \).
This section follows the nonparametric Bayes approach, that is, 
the data \( \Yv \) are described by the equation \( \Yv = \fvs + \epsv \)
for a fixed \( \fvs \).

Consider the situation with a family of Gaussian priors of the form
 \( \ND(0,\GP^{-2}) \) for a Gaussian regression model 
\( \Yv = \Psi^{\T} \thetav + \sigma \epsv \).
The corresponding penalized log-likelihood reads (up to a fixed constant)
\begin{EQA}
	L_{\GP}(\thetav)
	& \eqdef &
	- \frac{\bigl\| \Yv - \Psi^{\T} \thetav \bigr\|^{2}}{2 \sigma^{2}} 
	- \frac{\| \GP \thetav \|^{2}}{2} 
	+ \log \det \GP \, .
\label{LGtYvPT22fG22}
\end{EQA}
Consider a family of prior covariances
\( \bigl\{ \GP_{\hyper}^{-2} \bigr\} \) indexed by parameter \( \hyper \in \MM \).
% with covariances \( \GP^{-2} \) and \( \GP_{1}^{-2} \).
The full or hierarchical Bayes approach assumes that an additional prior \( \priorh \) is put on the hyperparameter 
\( \hyper \) taking value in the set of priors \( \MM \).
In what follows we assume that this set is discrete and 
denote \( \priorh_{\hyper} = \priorh(\GP_{\hyper}) \).
Also we write subindex \( \hyper \) in place of \( \GP_{\hyper} \) for ease of notation.
In particular, \( L_{\hyper}(\thetav) \) means \( L_{\GP_{\hyper}}(\thetav) \)
and \( \tilde{\thetav}_{\hyper} = \argmax_{\thetav} L_{\hyper}(\thetav) \).
It holds
\begin{EQA}
	\Yv 
	\cond 
%	\thetav, \hyper
%	\propto 
%	\exp\bigl\{ \LGP(\thetav) - \log \det \GP \bigr\} ,
%	\\
%	\Yv 
%	& \cond &
	\thetav, \hyper
	&\propto & 
	\exp\bigl\{ L_{\hyper}(\thetav) \bigr\} .
\label{YtGeLGldG11}
\end{EQA}
The full posterior writes
\begin{EQA}
	\thetav, \hyper \cond \Yv
	& \propto &
	\exp\bigl\{ L_{\hyper}(\thetav) \bigr\} 
		\priorh_{\hyper} \, .
%			{\exp\bigl\{ \LGP(\thetav) - \log \det \GP \bigr\} \priorh(\GP)
%	+ \exp\bigl\{ L_{\GP_{1}}(\thetav) - \log \det \GP_{1} \bigr\} \priorh(\GP_{1})}
\label{tapeLGaldGapGa}
\end{EQA}
The posterior of the hyperparameter \( \hyper \) is obtained by integration w.r.t. \( \thetav \):
\begin{EQA}
	\hyper \cond \Yv
	& \sim &
	\frac{\priorh_{\hyper} \int \exp\bigl\{ L_{\hyper}(\thetav) \bigr\} d\thetav}
		 {\sum_{\hyper \in \MM} \priorh_{\hyper} 
		 	\int\exp\bigl\{ L_{\hyper}(\thetav) \bigr\} d\thetav } \, .
\label{hYpGaieLGlddt}
\end{EQA}
%
The next result provides a useful representation for the hyperposterior. 
First we introduce some notations.
Let \( \fvs = \E \Yv \).
Let also \( \hyper \in \MM \) be fixed.
Define \( \BB_{\hyper} \eqdef \DPc \DP_{\hyper}^{-2} \DPc \)
\begin{EQA}
	\penm_{\hyper}
	& \eqdef &
	- \log\frac{\det \GP_{\hyper}^{2}}{\det \DP_{\hyper}^{2}} 
	=
	- \log \det (\Id - \BB_{\hyper}) \, ,
	\\
	\Pi_{\hyper} 
	&=& 
	\Psi^{\T} \bigl( \Psi \Psi^{\T} + \sigma^{2} \GP_{\hyper}^{2} \bigr)^{-1} \Psi ,
	\\
	\bias_{\hyper}^{2}
	&=&
	\bias_{\hyper}^{2}(\fvs)
	\eqdef 
%	\sigma^{-2} \| \fvs - \Pi_{\hyper} \fvs \|^{2} + \bigl\| \GP \thetavsGP \bigr\|^{2} 
%	=
	\sigma^{-2} \bigl\langle \fvs, (\Id - \Pi_{\hyper}) \fvs \bigr\rangle .
\label{bf2sm2fPih2}
\end{EQA} 
The use of elementary inequality \( - \log (1 - x) \geq x + x^{2}/2 \) for
\( x > 0 \) yields with \( \dimA_{\hyper}= \tr\bigl( \BB_{\hyper} \bigr) \) that
\begin{EQA}
	\varA_{\hyper}^{2}
	& \eqdef &
	\penm_{\hyper} - \dimA_{\hyper} 
	=
	- \log\frac{\det \GP_{\hyper}^{2} }{\det \DP^{2}_{\hyper}} 
	- \tr\bigl( \BB_{\hyper} \bigr)
	\\
	&=& 
	- \log \det \bigl\{ \Id - \DPc \DP_{\hyper}^{-2}  \DPc \bigr\}
	- \tr\bigl( \DPc \DP_{\hyper}^{-2}  \DPc \bigr)
	\geq 
	\frac{1}{2} \tr\bigl( \BB_{\hyper}^{2} \bigr)\, .
\label{12m12m12pAkm}
\end{EQA}
Finally denote for \( \tilde{\thetav}_{\hyper} = \argmax_{\thetav} L_{\hyper}(\thetav) = \bigl( \Psi \Psi^{\T} + \sigma^{2} \GP_{\hyper}^{2} \bigr)^{-1} \Psi \Yv \)
\begin{EQA}
	\risktt_{\hyper}
	& \eqdef &
	- L_{\hyper}(\tilde{\thetav}_{\hyper}) + {\penm_{\hyper}} /2,
%	+ \log (1/\priorh_{\hyper}) \, ,
	\\
	\riskt_{\hyper}
	& \eqdef &
	(\varA_{\hyper}^{2} + \bias_{\hyper}^{2})/2 ,
%	+ \log (1/\priorh_{\hyper}) \, ,
	\\
	\xiv_{\hyper} 
	& \eqdef & 
	\sigma^{-2} \DP_{\hyper}^{-1} \Psi \epsv
	=
	\sigma^{-1} \bigl( \Psi \Psi^{\T} + \sigma^{2} \GP_{\hyper}^{2} \bigr)^{-1/2} \Psi \epsv .
\label{evsm1PPTs2Fk2}
\end{EQA}

\begin{theorem}
\label{Thyperpost2}
Let \( \fvs = \E \Yv \) and \( \epsv = \Yv - \fvs \).
It holds
\begin{EQA}
	\hyper \cond \Yv
	& \sim &
	\frac{\exp\bigl( - \risktt_{\hyper} \bigr) \priorh_{\hyper}}
		 {\sum_{\hyper \in \MM} \exp\bigl( - \risktt_{\hyper} \bigr) \priorh_{\hyper}} 
	=
	\frac{\exp\bigl( - \riskt_{\hyper} + \zeta_{\hyper} \bigr) \priorh_{\hyper}}
		 {\sum_{\hyper \in \MM} \exp\bigl( - \riskt_{\hyper} + \zeta_{\hyper} \bigr) \priorh_{\hyper}} 
	\, 
\label{hcYcGapGaLGa22}
\end{EQA}
with
\begin{EQA}
	\zeta_{\hyper}
	& \eqdef & 
	\frac{1}{2} \bigl( 
		\bigl\| \xiv_{\hyper} \bigr\|^{2} - \E \bigl\| \xiv_{\hyper} \bigr\|^{2} 
	\bigr)
	- \sigma^{-2} \bigl\langle \epsv, \fvs - \Pi_{\hyper} \fvs \bigr\rangle .
\label{12s2Ee22lrfde}
\end{EQA}
\end{theorem}


This representation explains how the hyperposterior 
\( \hyper \cond \Yv \) behaves. 
Namely, suppose for a moment that the stochastic terms \( \zeta_{\hyper} \)
in \eqref{hcYcGapGaLGa22} vanish.
Then the  
hyperposterior \( \hyper \cond \Yv \) mainly concentrates on the model \( \hyper \) for which 
\( \riskt_{\hyper} \) is minimized.
In particular, for a uniform non-informative hyperprior with 
\( \priorh_{\hyper} \equiv \CONST \), the posterior is concentrated 
on the values \( \hyper \) that minimize the sum
\( \varA_{\hyper}^{2} + \bias_{\hyper}^{2} \).
This sum can be viewed as the bias-variance decomposition of the quadratic risk. 
%
In general, the stochastic terms \( \zeta_{\hyper} \) do not vanish but 
one can bound them in a uniform manner. 

%Introduce the subset \( \MMs_{\priorh} \subset \MM \) on which the value
%\( \riskt_{\hyper} \) is minimized:
%\begin{EQA}
%	\MMs_{\priorh}
%	& \eqdef &
%	\bigl\{ \hypers \in \MM \colon 
%		\riskt_{\hypers} = \min_{\hyper} \riskt_{\hyper}
%	\bigr\} .
%\label{MMspihsrklpk}
%\end{EQA} 
Introduce the index \( \hypers \subset \MM \) on which the value
\( \riskt_{\hyper} \) is minimized.
For ease of notation, assume that \( \hypers \) is uniquely defined. 
\begin{EQA}
	\hypers
	& \eqdef &
	\argmin_{\hyper} \riskt_{\hyper} \, .
\label{MMspihsrklpk}
\end{EQA} 
For any pair \( \hyper, \hyperm \in \MM \) and a fixed value \( \xx \), 
define 
\begin{EQA}
	\bias_{\hyper,\hyperm}^{2} 
	&=& 
	\sigma^{-2} \bigl| \bigl\langle \fvs, (\Pi_{\hyper} - \Pi_{\hyperm}) \fvs \bigr\rangle \bigr| ,
	\\
	\BB_{\hyper,\hyperm}
	& \eqdef &
	\DPc \bigl( \DP_{\hyper}^{-2} - \DP_{\hyperm}^{-2} \bigr) \DPc,
\label{bikk2vakksm2}
\end{EQA}
and 
%with \( \BB_{\hyper,\hyperm} \eqdef \DPc \bigl( \DP_{\hyper}^{-2} - \DP_{\hyperm}^{-2} \bigr) \DPc \)
\begin{EQ}[rcl]
	\vA_{\hyper,\hyperm}^{2}
	\eqdef
	\tr \BB_{\hyper,\hyperm}^{2} ,
	& \quad &
	\lambda_{\hyper,\hyperm}
	\eqdef 
	\lambda_{\max}(\BB_{\hyper,\hyperm}) .
\label{bikk2vakk222}
\end{EQ} 
For any \( \xx > 0 \), 
denote
\begin{EQA}
	\disth_{\hyper,\hyperm}(\xx)
	&=&
	\bigl( \bias_{\hyper,\hyperm} \, \sqrt{2\xx} 
	+ \vA_{\hyper,\hyperm} \sqrt{\xx}
	+ \lambda_{\hyper,\hyperm} \xx \bigr) .
\label{dks2xbksvksxxx}
\end{EQA}
The increments \( \risktt_{\hyper,\hypers} = \risktt_{\hyper} - \risktt_{\hypers} \)
of the process \( \risktt_{\hyper} \) can be well approximated by its expectation
\( \riskt_{\hyper,\hypers} \) in the sense that 
\( \bigl| \risktt_{\hyper,\hypers} - \riskt_{\hyper,\hypers} \bigr| > \disth_{\hyper,\hypers}(\xx) \)
only with a very small probability of order \( \ex^{-\xx} \).

\begin{theorem}
\label{TupperfR}
Let \( \hypers \) %\( \MMs_{\priorh} \) 
be defined in \eqref{MMspihsrklpk}.
%Let a sequence \( \zz_{\hyper,\hypers} \) be fixed such that
%\( \sum_{\hyper \in \MM} \exp ( - \zz_{\hyper,\hypers} ) \leq 1 \).
Then on a random set \( \Omega(\xx) \) with \( \P\bigl( \Omega(\xx) \bigr) \geq 1 - 3 \ex^{-\xx} \),
it holds
\begin{EQA}
	\bigl| \riskt_{\hyper,\hypers} - \risktt_{\hyper,\hypers} \bigr|
	& \leq &
	\disth_{\hyper,\hypers} \, ,
	\quad
	\hyper \in \MM .
\label{RRtkkthMM}
\end{EQA}
with %\( \xx_{\hyper} = \xx + \log(1/\priorh_{\hyper}) \).
\begin{EQA}
	\disth_{\hyper,\hypers}
	&=&
	\disth_{\hyper,\hypers}(\xx + \log\priorh_{\hyper}^{-1}) .
\label{dgkstxlpk1}
\end{EQA}
%
%
\end{theorem}

An immediate corollary of this uniform bound is the concentration property of the posterior.
We show that the hyperposterior concentrates in a \( \disth \)-vicinity of \( \hypers \).
%\( \MMs_{\priorh} \). 
More specifically, if 
\( \riskt_{\hyper} - \riskt_{\hypers} \gg \disth_{\hyper,\hypers} \) 
%for some \( \hypers \in \MMs_{\priorh} \)
then the posterior probability of \( \hyper \) is negligible. 
For any subset \( \MA \subset \MM \), define
\begin{EQA}
	\priorhu(\MA)
	& \eqdef &
	\sum_{\hyper \in \MA} \priorh_{\hyper} 
	\exp\bigl( - \riskt_{\hyper,\hypers} + \disth_{\hyper,\hypers} \bigr),
	\\
	\priorhd(\MA)
	& \eqdef &
	\sum_{\hyper \in \MA} \priorh_{\hyper} 
	\exp\bigl( - \riskt_{\hyper,\hypers} - \disth_{\hyper,\hypers} \bigr),
\label{pipluspimiAghht}
\end{EQA}

\begin{theorem}
\label{Tpostcontpr}
The posterior probability \( \priorh(\MA \cond \Yv) \) of any \( \MA \subset \MM \) fulfills
on a random set \( \Omega(\xx) \) with \( \P\bigl( \Omega(\xx) \bigr) \geq 1 - 3 \ex^{-\xx} \)
\begin{EQA}[rcccl]
	\frac{\priorhd(\MA)}{\priorhd(\MA) + \priorhu(\MM \backslash \MA)}
	& \leq &
	\priorh(\MA \cond \Yv )
	& \leq &
	\frac{\priorhu(\MA)}{\priorhu(\MA) + \priorhd(\MM \backslash \MA)}
\label{Memxrtrtsdhk}
\label{MexEpMdsYdks}
\end{EQA}
\end{theorem}
	
\begin{corollary}
\label{CTpostcontpr}
Let 
\begin{EQA}
	\frac{\priorhu(\MM \backslash \MA)}{\priorhd(\MA)}
	&Ê\leq &
	\alp. 
\label{fpaMmAMAa}
\end{EQA}
Then 
\begin{EQA}
	\priorh(\MA \cond \Yv )
	&Ê\geq &
	1 - \alp. 
\label{fpaMmAMAa1a}
\end{EQA}
\end{corollary}

The properties of the posterior measure \( \priorh(\hyper \cond \Yv) \) are difficult to study, 
because of its nature as a normalized sum of random exponents. 
Now we introduce another deterministic measure \( \priorhb(\hyper) \) and show that these two measure are 
close to each other, e.g., w.r.t. the Kullback-Leibler divergence.
Define for \( \hyper \in \MM \)
\begin{EQA}
	\risktm_{\hyper,\hypers}
	& \eqdef &
	\riskt_{\hyper,\hypers} - \disth_{\hyper,\hypers} \, ,
	\\
	\priorhb(\hyper)
	& \eqdef &
	\frac{\exp \bigl( - \risktm_{\hyper,\hypers} \bigr) \priorh_{\hyper}}
		 {\sum_{\hyper \in \MM} \exp \bigl( - \risktm_{\hyper,\hypers} \bigr) \priorh_{\hyper}} \, .
\label{phbdefmRthrt}
\end{EQA}
Define also the ratio 
\begin{EQA}
	Z(\hyper)
	& \eqdef &
	\frac{\priorh(\hyper \cond \Yv)}{\priorhb(\hyper)} \, .
\label{ZkkfpakAY}
\end{EQA}

\begin{theorem}
\label{TKLpriorhhb}
Let \( \disth_{\hyper,\hypers} \) be defined in \eqref{dgkstxlpk1}. 
Then it holds on a random set \( \Omega(\xx) \) for any positive monotonous function \( f(z) \)
with \( f(1) = 1 \)
\begin{EQA}
	\E_{\priorhb} f(Z)
	&Ê\leq &
	\E_{\priorhb} f(2 \disth_{\hyper,\hypers})
\label{EfZEf2dkks}
\end{EQA}
\begin{EQA}
	\kullb\bigl( \priorhb, \priorh(\Yv) \bigr)
	& \leq &
	2 \E_{\priorhb} \, \disth_{\hyper,\hypers} .
\label{KLphbphY}
\end{EQA}
\end{theorem}

\begin{proof}
Denote \( \risktt_{\hyper,\hypers} = \risktt_{\hyper} - \risktt_{\hypers} \).
We use that
\begin{EQA}
	\risktt_{\hyper,\hypers} - \risktm_{\hyper,\hypers}
	&=&
	\distht_{\hyper,\hypers} + \disth_{\hyper,\hypers}
	\in 
	[0,2\disth_{\hyper,\hypers}]
\label{rrkksmRkks02}
\end{EQA}
on \( \Omega(\xx) \).
This implies by definition of \( \priorhb \)
\begin{EQA}
	\kullb\bigl( \priorhb, \priorh(\Yv) \bigr)
	&=&
	\sum_{\hyper \in \MM} \priorhb(\hyper) \log \frac{\priorhb(\hyper)}{\priorh(\hyper \cond \Yv)}
	\\
	&=&
	\sum_{\hyper \in \MM} \bigl( \risktt_{\hyper,\hypers} - \risktm_{\hyper,\hypers} \bigr)\priorhb(\hyper) 
	+ \log \frac{\sum \exp(- \risktt_{\hyper,\hypers})}{\sum \exp(- \risktm_{\hyper,\hypers})}
	\\
	&=&
	\sum_{\hyper \in \MM} \bigl( \risktt_{\hyper,\hypers} - \risktm_{\hyper,\hypers} \bigr)\priorhb(\hyper) 
	+ \log \sum_{\hyper \in \MM} \exp\bigl( - \risktt_{\hyper,\hypers} + \risktm_{\hyper,\hypers} \bigr) \priorhb(\hyper)
	\\
	& \leq &
	2 \sum_{\hyper \in \MM} \disth_{\hyper,\hypers} \, \priorhb(\hyper) 
	+ \log \sum_{\hyper \in \MM} \priorhb(\hyper) 
	=
	2 \E_{\priorhb} \, \disth_{\hyper,\hypers} \, ,
\label{kMfdkmldkmf}
\end{EQA}
and the result follows.
\end{proof}


\begin{remark}
The result \eqref{KLphbphY} is meaningful if the quantity 
\( \E_{\priorhb} \, \disth_{\hyper,\hypers} \) is sufficiently small. 
The definition of \( \priorhb \) yields that the this measure well concentrates on a small vicinity of \( \hypers \).
This easily implies ???
\end{remark}

The bound \eqref{KLphbphY} is useful in combination with the following technical result 
known as ``information theoretic bound''.

\begin{lemma}[\cite{Sp2009}, Lemma 2.6]
\label{LTIB}
Let \( \P \) and \( \P_{0} \) be two measures such that \( \E \log(d\P/d\P_{0}) < \infty \). 
Then, for any random variable \( \zeta \) with \( \E_{0} \zeta < \infty \), it holds
\begin{EQA}
	\E \log(1 + \zeta)
	& \leq &
	\E \log(d\P/d\P_{0}) + \E_{0} \zeta .
\label{El1zElPP0z}
\end{EQA}
\end{lemma}

\begin{theorem}
\label{Tcontpostappr}
Let \( \xi(\hyper) = \xi(\hyper,\Yv) \) be any family of loss functions.
Then on a random set \( \Omega(\xx) \), it holds after the plug-in the posterior 
\( \priorh \cond \Yv \)
\begin{EQA}
	\log \left( 1 + \sum \xi(\hyper) \priorh(\hyper \cond \Yv ) \right)
	&=&
	\sum \priorhb(\hyper) \, \xi(\hyper)
%	\log(2) \, \priorh\bigl( \MM_{\alp} \cond \Yv \bigr)
%	&Ê\leq &
  	+ 2 \E_{\priorhb} \, \disth_{\hyper,\hypers} \, . 
\label{l1sxikkcYdkks}
\end{EQA}
\end{theorem}

\begin{proof}
We apply Lemma~\ref{LTIB} to \( \zeta(\hyper) = c \Ind_{\MM_{\alp}}(\hyper) \). 
The result follows from  Theorem~\ref{TKLpriorhhb} in view of 
\( \log(1 + \zeta) = \log(2) \, \zeta \).
\end{proof}

\subsection{Iterated hierarchical prior}
A natural idea for selecting the hyperprior is to start with a uniform non-informative hyperprior 
and then to use the hyperposterior as a hyperprior once again. 

Define a vicinity of \( \hypers \) by the relation
\begin{EQA}
	\MM(\xx)
	&\eqdef &
	\bigl\{ 
		\riskt_{\hyper} - \riskt_{\hypers} \leq	\disth_{\hyper,\hypers}(\xx) 
	\bigr\} .
\label{¥}
\end{EQA}
We know from Theorem~\ref{TupperfR} that \( \xx \) larger than \( \xx_{1} = \xx_{0} + \log (\#\MM) \) ensures that the posterior 
concentrates on \( \MM(\xx_{1}) \) with probability at least \( 1 - \ex^{-\xx_{0}} \).
Now we aim at refining this result by reducing the value \( \xx_{1} \) to the 
\( \xx_{2} = \xx_{0} + \log \bigl( \# \MM(\xx_{1}) \bigr) \).
Define
\begin{EQA}
	\priorh_{1}(\hyper)
	& \propto &
	\exp \bigl( - \risktt_{\hyper} \bigr) \priorh_{0}(\hyper)
	=
	\frac{\exp \bigl( - \risktt_{\hyper} \bigr) \priorh_{0}(\hyper)}
		 {\sum_{\hyper \in \MM} \exp \bigl( - \risktt_{\hyper} \bigr) \priorh_{0}(\hyper)}
\label{¥}
\end{EQA}
Further, recompute the posterior
\begin{EQA}
	\priorh_{2}(\hyper)
	& \propto &
	\exp \bigl( - \risktt_{\hyper} \bigr) \priorh_{1}(\hyper)
	=
	\frac{\exp \bigl( - \risktt_{\hyper} \bigr) \priorh_{1}(\hyper)}
		 {\sum_{\hyper \in \MM} \exp \bigl( - \risktt_{\hyper} \bigr) \priorh_{1}(\hyper)} .
\label{¥}
\end{EQA}

%Define \( \priorh_{0}(\hyper) = (\#\MM)^{-1} \) and 
%\begin{EQA}
%	\priorhp_{0}(\hyper)
%	& \propto &
%	\exp \bigl( - \risktt_{\hyper} \bigr) \priorh_{0}(\hyper)
%	=
%	\frac{\exp \bigl( - \risktt_{\hyper} \bigr) \priorh_{0}(\hyper)}
%		 {\sum_{\hyper \in \MM} \exp \bigl( - \risktt_{\hyper} \bigr) \priorh_{0}(\hyper)}
%\label{¥}
%\end{EQA}
%and set
%\begin{EQA}
%	\priorh_{1}(\hyper)
%	&=&
%	\priorhp_{0}(\hyper) \Ind\bigl( \priorhp_{0}(\hyper) \geq \ex^{-\xx_{0}} \bigr) .
%\label{¥}
%\end{EQA}
%Further, recompute the posterior
%\begin{EQA}
%	\priorhp_{1}(\hyper)
%	& \propto &
%	\exp \bigl( - \risktt_{\hyper} \bigr) \priorh_{1}(\hyper)
%\label{¥}
%\end{EQA}
%and apply thresholding
%\begin{EQA}
%	\priorh_{2}(\hyper)
%	&=&
%	\priorhp_{1}(\hyper) \Ind\bigl( \priorhp_{1}(\hyper) \geq \ex^{-\xx_{0}} \bigr) .
%\label{¥}
%\end{EQA}
%If necessary, iterate until convergence.
Theorem~\ref{¥}


\subsection{Max-Bayes approach}
This section provides another viewpoint on the problem of Bayesian model selection.
The main difference is in the assumption on the true data generating process.
Namely, we consider the model \( \Yv = \fvs + \epsv \) but assume that 
%\( \fvs \) follows a prior \( \ND(0,\GP_{\hyperu}^{-2}) \), that is,
\( \fvs = \Psi^{\T} \thetav \) and \( \thetav \sim \ND(0,\GP_{\hyperu}^{-2}) \).
By \( \P_{\hyperu} \) we denote the corresponding joint distribution of 
\( \Yv \) and \( \thetav \).
First we consider the case when \( \hyperu \) belongs
to a given family \( \bigl( \GP_{\hyper}, \, \hyper \in \MM \bigr) \).
%Note that we do not require \( \hyperu \in \MM \).
We are interested to establish sufficient conditions which ensure 
a concentration of the hyperposterior in a vicinity of \( \hyperu \).
The key observation is that the squared bias
\( \bias_{\hyper}^{2}(\fvs) = \bias_{\hyper}^{2}(\Psi^{\T} \thetav) \) 
concentrates around some fixed value when 
\( \thetav \sim \ND(0,\GP_{\hyperu}^{-2}) \).
More specifically, for each \( \hyper \in \MM \), 
the squared bias can be written as
\begin{EQA}
%	\biasm^{2}_{\hyper \| \hyperu}
%	=
	\bias_{\hyper}^{2}(\Psi^{\T} \thetav) 
%	- \bias_{\hyperu}^{2}(\Psi^{\T} \thetav)
	&=&
	\sigma^{-2} \bigl\langle \thetav, \Psi (\Id - \Pi_{\hyper})
%	(\Pi_{\hyperu} - \Pi_{\hyper}) 
	\Psi^{\T} \thetav \bigr\rangle .
\label{s2b2kfsIPfPPT}
\end{EQA} 
Now we replace \( \thetav \) with \( \GP_{\hyperu}^{-1} \gammav \),
where \( \gammav \) is standard normal in \( \R^{\dimp} \).
Therefore, the squared bias is a Gaussian quadratic form 
\( \bigl\langle \BB_{\hyper \| \hyperu} \gammav, \gammav \bigr\rangle \)
with
\begin{EQA}
	\BB_{\hyper \| \hyperu}
	& \eqdef &
	\sigma^{-2} \GP_{\hyperu}^{-1} \Psi 
%	(\Pi_{\hyperu} - \Pi_{\hyper}) 
	(\Id - \Pi_{\hyper})
	\Psi^{\T} \GP_{\hyperu}^{-1} 
	=
	\GP_{\hyperu}^{-1} \bigl( \Id - \DPc^{2} 
%	(\DP_{\hyperu}^{-2} - \DP_{\hyper}^{-2}) 
	\DP_{\hyper}^{-2}
	\DPc^{2} \bigr) \GP_{\hyperu}^{-1}.
\label{Bkmsm2Dm1Pikm1}
\end{EQA}
Concentration of Gaussian quadratic forms allows to approximate 
this quadratic form by its expectation \( \tr \BB_{\hyper \| \hyperu} \); see
Theorem~\ref{TexpbLGA}.
Therefore, for the uniform non-informative hyperprior \( \priorh \), define for each \( \hyper \in \MM \) the risk
\begin{EQA}
	\riskt_{\hyper \| \hyperu}
	& \eqdef &
	\frac{1}{2} 
	\bigl( \varA_{\hyper}^{2} + \tr \BB_{\hyper \| \hyperu} \bigr) .
%	+ \log \priorh_{\hyper} - \log \priorh_{\hyperu}\, .
\label{rkmde12vkvamt}
\end{EQA}

\begin{lemma}
\label{LmaxBayes}
Let \( \hyperu \in \MM \).
It holds
\begin{EQA}
	\hyperu
	&=&
	\argmin_{\hyper \in \MM} \riskt_{\hyper \| \hyperu} .
\label{hmakRkmM2k12}
\end{EQA}
\end{lemma}

\begin{proof}
To be checked that \( \riskt_{\hyperu \| \hyperu} - \riskt_{\hyper \| \hyperu} \) is the KL divergence between 
\( \P_{\hyperu} \) and \( \P_{\hyper} \).
\end{proof}

To state the result about concentration of the hyperposterior, 
consider the relative bias \( \bias_{\hyper}^{2}(\Psi^{\T} \thetav) - \bias_{\hyperu}^{2}(\Psi^{\T} \thetav) \).
It can be represented as 
\begin{EQA}
	\bias_{\hyper}^{2}(\Psi^{\T} \thetav) - \bias_{\hyperu}^{2}(\Psi^{\T} \thetav)
	& \eqdef &
	\bigl\langle (\BB_{\hyper \| \hyperu} - \BB_{\hyperu \| \hyperu}) \gammav, \gammav \bigr\rangle
	=
	\bigl\langle \BBB_{\hyper \| \hyperu} \gammav, \gammav \bigr\rangle
\label{bm2kmBkmtBk}
\end{EQA}
with \( \BBB_{\hyper \| \hyperu} = \BB_{\hyper \| \hyperu} - \BB_{\hyperu \| \hyperu} \).
Theorem~\ref{TexpbLGA} about concentration of Gaussian quadratic forms
 helps to bound its deviation from expectation:
\begin{EQA}
	\P_{\hyperu}\Bigl( 
		\Bigl| \bigl\langle \BBB_{\hyper \| \hyperu} \gammav, \gammav \bigr\rangle - \tr (\BBB_{\hyper \| \hyperu}) \Bigr|
		> 2 \vA_{\hyper \| \hyperu} \sqrt{\xx} 
		+ 2 \lambda_{\hyper \| \hyperu} \, \xx 
	\Bigr)
	& \leq &
	\ex^{-\xx} ,
\label{vAkmsx2xdkm}
\end{EQA}
where 
\begin{EQA}
	\vA^{2}_{\hyper \| \hyperu} 
	\eqdef 
	\tr (\BBB^{2}_{\hyper \| \hyperu}) 
	=
	\| \BBB_{\hyper \| \hyperu} \|_{\Fr}^{2} \, ,
	& \qquad &
	\lambda_{\hyper \| \hyperu} 
	\eqdef 
	\| \BBB_{\hyper \| \hyperu} \| \, .
\label{trBkm2kmvAkm2}
\end{EQA}
Define for \( \vA_{\hyper,\hyperu} \, , \lambda_{\hyper,\hyperu} \) from \eqref{bikk2vakk222} and \( \vA_{\hyper \| \hyperu}, \lambda_{\hyper \| \hyperu} \) from \eqref{trBkm2kmvAkm2}
\begin{EQA}
	\disth_{\hyper \| \hyperu}
	& \eqdef &
	\Bigl( \vA_{\hyper \| \hyperu} + \vA_{\hyper,\hyperu} 
		+ 2 \sqrt{\tr \bigl( |\BBB_{\hyper \| \hyperu}| \bigr)}
	\Bigr) \sqrt{\xx_{\hyper}} 
	+ \bigl( \lambda_{\hyper \| \hyperu} 
	+ \lambda_{\hyper,\hyperu} \bigr) \xx_{\hyper}
\label{dkmVkmsx2x}
\end{EQA}
%and introduce the set \( \MMd_{\hyperu} \) 
%\begin{EQA}
%	\MMd_{\hyperu}
%	& \eqdef &
%	\bigl\{ \hyper \colon
%	\riskt_{\hyper \| \hyperu} - \riskt_{\hyperu \| \hyperu}
%	\geq 
%%	\disth_{\hyper,\hyperm} + 
%	\disth_{\hyper \| \hyperu} \bigr\} .
%\label{MMmkmdkmdk2mx}
%\end{EQA}
%Here \( \disth_{\hyper,\hyperm} \) is from \eqref{dks2xbksvkssx}.
%
Also define for \( \MA \subset \MM \)
\begin{EQA}
	\priorhu_{\hyperu}(\MA)
	& \eqdef &
	\sum_{\hyper \in \MA} \priorh_{\hyper} 
	\exp\bigl( - \riskt_{\hyper \| \hyperu} +  \riskt_{\hyperu \| \hyperu} + \disth_{\hyper \| \hyperu} \bigr),
	\\
	\priorhd_{\hyperu}(\MA)
	& \eqdef &
	\sum_{\hyper \in \MA} \priorh_{\hyper} 
	\exp\bigl( - \riskt_{\hyper \| \hyperu} + \riskt_{\hyperu \| \hyperu} - \disth_{\hyper \| \hyperu} \bigr),
\label{pivpluspivmiAghht}
\end{EQA}

\begin{theorem}
\label{TmaxBayescontraction}
Let \( \Yv = \Psi^{\T} \thetav + \epsv \) and 
\( \thetav \sim \ND(0,\GP_{\hyperu}^{-2}) \) for some \( \hyperu \in \MM \).
Consider a hyperprior \( \priorh \).
Then on a set \( \Omega(\xx) \) with \( \P_{\hyperu}\bigl( \Omega(\xx) \bigr) \geq 1 - 5 \ex^{-\xx} \), it holds
\begin{EQA}[rcccl]
	\frac{\priorhd_{\hyperu}(\MA)}{\priorhu_{\hyperu}(\MA) + \priorhd_{\hyperu}(\MM \backslash \MA)}
	& \leq &
	\priorh(\MA \cond \Yv )
	& \leq &
	\frac{\priorhd_{\hyperu}(\MA)}{\priorhu_{\hyperu}(\MA) + \priorhu_{\hyperu}(\MM \backslash \MA)} \, .
\label{MemxrtrtsdhkBx}
\end{EQA}
\end{theorem}


\begin{remark}
Suppose that the set \( \MA \) consists of just one point \( \hyperu \).
%If \( \hyperu \in \MM \), then this point is \( \hyperu \) by Lemma~\ref{LmaxBayes}.
Then we obtain a kind of ``sharp adaptive'' or ``oracle adaptive'' result:
the hyperposterior concentrates on the true model. 
By definition of \( \MMd_{\hyperu} \), it suffices to ensure that 
\( \riskt_{\hyper \| \hyperu} \geq \riskt_{\hyperu \| \hyperu} + \disth_{\hyper \| \hyperu} \) 
for \( \hyper \neq \hyperu \) 
to get \( \priorh(\MMd_{\hyperu} \cond \Yv ) \leq \alp \) on a set of dominating probability.
\end{remark}

Finally we extend the result of Theorem~\ref{TKLpriorhhb}.
Define the measure \( \priorhb \) on \( \MM \) by
\begin{EQA}
	\priorhb(\hyper)
	& \eqdef &
	\frac{\exp \bigl( - \riskt_{\hyper} + \riskt_{\hypermu} \bigr) \priorh_{\hyper}}
		 {\sum \exp \bigl( - \riskt_{\hyper} + \riskt_{\hypermu} \bigr) \priorh_{\hyper}}  \, .
\label{phbdefmRthrt}
\end{EQA}

\begin{theorem}
\label{TKLpriorhhbpr}
Under conditions of Theorem~\ref{TmaxBayescontractionpi}, 
it holds on a random set \( \Omega(\xx) \) with \( \P_{\hyperu} \geq 1 - 5 |\MM| \ex^{-\xx} \)
\begin{EQA}
	\kullb\bigl( \priorhb, \priorh(\Yv) \bigr)
	& \leq &
	2 \log \E_{\priorhb} \exp \disth_{\hyper,\hypers} .
\label{KLphbphYpr}
\end{EQA}
\end{theorem}



\subsection{Ordered hyperpriors}
\label{Sorderedhyper}
%The aim of this section is to justify a reasonable choice of the hyperprior \( \priorh \) yielding 
%a posterior with prescribed properties.
%Now we explain the approach for selecting the hyperprior by the so called propagation condition.
Suppose that the set of prior covariances \( \bigl\{ \GP_{\hyper}^{2}, \hyper \in \MMs \bigr\} \) is ordered
by the univariate hyperparameter \( \hyper \) in the sense that
\begin{EQA}
	\GP_{\hyper}^{2}
	& \leq &
	\GP_{\hyperc}^{2} ,
	\quad
	\hyperc \geq \hyper .
\label{GPorderhh2}
\end{EQA}
The larger index \( \hyper \), the weaker penalization induced by \( \GP_{\hyper}^{2} \).
The effective dimension 
\( \dimA_{\hyper} = \tr \BB_{\hyper} = \tr\bigl( \DPc^{2} \DP_{\hyper}^{-2} \bigr) \) and the variance term \( \varA_{\hyper}^{2} \) increase with \( \hyper \) as well.
The set \( \MMs \) can be continuous or countable.
We build a proper finite subset \( \MM \) of \( \MMs \) and use it as a non-informative hyperprior
which ensures a sharp adaptive result in Bayesian model selection.
Without loss of generality we can write \( \MM = \bigl\{ 1,\ldots, \mmmax \bigr\} \)
and 
\begin{EQA}[c]
	\GP_{1}^{2} \geq \GP_{2}^{2} \geq \ldots \geq \GP_{\mmmax}^{2}    .
\label{G1G2G22dots}
\end{EQA}
Under the nonparametric Bayes approach 
with a fixed response \( \fvs = \E \Yv \), the squared bias term for the hyper value \( \hyper \) is given by the value \( \bias_{\hyper}^{2} = \bias_{\hyper}^{2}(\fvs) \);
see \eqref{bf2sm2fPih2}.
It obviously decreases with \( \hyper \).
The optimal prior choice \( \hypers \) corresponds to the minimum of the sum 
\( \riskt_{\hyper}(\fvs) = \bias_{\hyper}^{2}(\fvs) + \varA_{\hyper}^{2} \);
see \eqref{MMspihsrklpk}.

In the max-Bayes approach we assume \( \fvs = \Psi^{\T} \thetav \) and 
\( \thetav \sim \ND(0,\GP_{\hyperu}^{-2}) \),
the squared bias 
\( \bias_{\hyper}^{2}(\fvs) = \bias_{\hyper}^{2}(\Psi^{\T} \thetav) \) concentrates around its expectation 
\( \tr \BB_{\hyper \| \hyperu} \).
The optimal model choice is \( \hyperu \) if this model is in \( \MM \)
or the point \( \hypermu \in \MM \) closest to \( \hyperu \), see \eqref{mpiksakRpkks}.
Of interest is whether the full Bayes approach yields the sharp adaptive result. 
This will be the case if the hyperposterior concentrates on a singleton 
\( \hypermu \) from \eqref{mpiksakRpkks}.
A sufficient condition is given by Theorems~\ref{TmaxBayescontraction} and \ref{TmaxBayescontractionpi}: 
\( \riskt_{\hyper \| \hyperu} - \riskt_{\priorh}(\hypermu \| \hyperu)
	\geq \disth_{\hyper \| \hyperu} + \xx \) for all \( \hyper \in \MM \) such that
	\( \hyper \neq \hypermu \) and for 
\( \xx \) sufficiently large.
In other words, the set \( \MM \) should be discrete and distance between 
any two neighbor points is large enough.

We construct \( \MM \) step-by-step starting from the smallest model \( \hyper_{1} \).
The only requirement is that the corresponding effective dimension \( \dimA_{\hyper_{1}} \) is 
significantly larger than the standard deviation \( \vA_{\hyper_{1}} \).
Then we fix the closest value \( \hyper_{2} \in \MMs \) such that 
\begin{EQA}
	\riskt(\hyper_{2} \| \hyper_{1}) - \riskt(\hyper_{1} \| \hyper_{1})
	& \geq &
	\disth(\hyper_{2} \| \hyper_{1}) + \xx .
\label{r21r11d21x}
\end{EQA}
With \( \hyper_{1} < \hyper_{2} < \ldots < \hyper_{\mm} \) fixed, the next value \( \hyper_{\mm+1} \) is selected 
by the similar rule
\begin{EQA}
	\riskt(\hyper_{\mm+1} \| \hyper_{\mm}) - \riskt(\hyper_{\mm} \| \hyper_{\mm})
	& \geq &
	\disth(\hyper_{\mm+1} \| \hyper_{\mm}) + \xx 
\label{rm1rmmdm1x}
\end{EQA}
until we reach the largest value \( \hyper_{\max} \) in \( \MMs \).
The construction ensures that under \( \P_{\hyper_{\mm}} \), the posterior of the next largest model \( \hyper_{\mm+1} \)
will be smaller than \( \ex^{-\xx} \).
This easily yields that the posterior of the event \( \hyper > \hyper_{\mm} \) will be smaller than \( 2 \ex^{-\xx} \).

\begin{theorem}
\label{Tsharpadapt}
Let \( \mm_{1} \) be large enough to provide ???
Then for any \( \hypers \in \MMs \)
\begin{EQA}
	\E_{\hypers} \bigl\| \QP (\tilde{\thetav}_{\hyper} - \thetav) \bigr\|^{2}
	& \leq &
	\bigl( 1 + ??? \bigr)
	\E_{\hypers} \bigl\| \QP (\tilde{\thetav}_{\hypers} - \thetav) \bigr\|^{2}
\label{EkQQ1ttkt2}
\end{EQA}
\end{theorem}

%
%The relative bias \( \bias_{\hyper,\hypers}^{2} = \bias_{\hyper,\hypers}^{2}(\fvs) \) depends on the underlying truth \( \fvs \) and is not accessible. 
%However, we wish to build a hyperprior \( \priorh \) such that the posterior probability for 
%all larger models will be small. 
%We refer to this property as ``one-sided contraction''. 
%The aim is to find a hyperprior which is possibly close to a non-informative prior on the set 
%\( \MM \) but still ensures this contraction property.
%
%We build the hyperprior \( \priorh \) successively starting from the largest model in the family 
%\( \bigl\{ \GP_{\hyper} \bigr\} \).
%For each \( \hyperm \), define a subset 
%\( \MMu_{\mm} = \bigl\{ \mm,\ldots,\mmmax \bigr\} \subseteq \MM \).
%Suppose the prior \( \priorh_{\hyperm+1} \) on \( \MMu_{\mm+1} \) is already built.
%We explain how to extend this construction to the set \( \MMu_{\mm} \).
%For each value \( p_{\hyperm} \in [0,1] \), define the hyperprior \( \priorh_{\hyperm} \) on 
%\( \MMu_{\hyperm} \)
%with \( \priorh_{\hyperm}(\hyperm) = p_{\hyperm} \) and 
%\( \priorh_{\hyperm}(\hyper) = (1 - p_{\hyperm}) \priorh_{\hyperm+1}(\hyper) \), \( \hyper > \hyperm \).
%The hyperprior \( \priorh_{\hyperm}  \) yields a posterior \( \priorh_{\hyperm} \cond \Yv^{\synt} \)
%on \( \MMu_{\mm} \)
%assigning the mass \( \priorh_{\hyperm}(\hyper,\Yv^{\synt}) \) to each \( \hyper \geq \hyperm \).
%Our condition means that this posterior concentrates on \( \hyperm \) as long as \( \thetav \) comes
%from the model \( \hyperm \), that is, \( \thetav \sim \ND(0, \GP_{\hyperm}^{-2}) \).
%More precisely, define the smallest value \( p_{\hyperm} \) ensuring the propagation condition
%\begin{EQA}
%	\sum_{\hyper > \hyperm} %(1 - p_{\hyperm}) \priorh_{\hyperm+1}(\hyper)
%		\int \E_{\thetav} \priorh_{\hyperm}(\hyper, \Yv^{\synt}) \, 
%			\phi_{(0,\GP_{\hyperm}^{-2})}(\thetav) \, d\thetav
%	& \leq &
%	\ex^{-\xxm} .
%\label{iPPhG1cYpGd}
%\end{EQA}
%Here the values \( \xxm \) should satisfy \( \sum_{\hyperm} \ex^{-\xxm} = \ex^{-\xx} \).
%Given \( \xxm \), the value \( p_{\hyperm} \) and thus, the prior \( \priorh_{\hyperm} \) are uniquely defined. 
%This approach assumes that the set \( \MM \) is fixed in a way that the ``distance'' 
%between any two neighbor models \( \hyperm \) and \( \hyperm + 1 \) 
%is sufficiently large. 
%
%An alternative approach is to consider the averaged difference 
%\( \risktt_{\hyper} - \risktt_{\hyperm} \). 
%quadratic prediction risk
%\begin{EQA}
%	\E_{\thetav} \bigl\| \Psi^{\T} \bigl( \tilde{\thetav}_{\hyper} - \thetav \bigr) \bigr\|^{2}
%	&=&
%	\E_{\thetav} \bigl\| \Psi^{\T} \bigl( \tilde{\thetav}_{\hyper} - \thetav \bigr) \bigr\|^{2}
%	=
%	\bigl\| \Psi^{\T} \bigl( \thetavs_{\hyper} - \thetav \bigr) \bigr\|^{2} 
%	+ \tr \bigl( \DP^{2} \DP_{\hyper}^{-2} \bigr)
%	=
%	\bias_{\hyper}^{2}(\thetav) + \dimA_{\hyper}
%\label{EtEtPTttkt}
%\end{EQA}
%with \( \thetavs_{\hyper} = \thetavs_{\hyper}(\thetav) 
%= \bigl( \Psi \Psi^{\T} + \sigma^{2} \GP_{\hyper}^{2} \bigr)^{-1} \Psi \Psi^{\T} \thetav \).
%This value averaged over \( \thetav \sim \ND(0,\GP_{\hyperm}^{-2}) \), defines a kind of distance 
%between \( \hyper \) and \( \hyperm \) models.
%It holds 
%\begin{EQA}
%	\bias_{\hyper}^{2}(\hyperm)
%	\eqdef
%	E_{\thetav \sim \ND(0,\GP_{\hyperm}^{-2})} \bias_{\hyper}^{2}(\thetav)
%	& \eqdef &
%	\int  \, \bigl\| \Psi^{\T} \bigl( \thetavs_{\hyper} - \thetav \bigr) \bigr\|^{2}
%			\phi_{(0,\GP_{\hyperm}^{-2})}(\thetav) \, d\thetav
%	\\
%	&=&
%	\int  \, \bigl\| \bigl( \Id - \Pi_{\hyper} \bigr) \Psi^{\T} \thetav \bigr\|^{2}
%			\phi_{(0,\GP_{\hyperm}^{-2})}(\thetav) \, d\thetav
%	\\
%	&=&
%	\E \bigl\| \bigl( \Id - \Pi_{\hyper} \bigr) \Psi^{\T} \DP_{\hyperm}^{-1} \gammav \bigr\|^{2}
%	=
%	\tr \bigl\{ \bigl( \Id - \Pi_{\hyper} \bigr) \Psi^{\T} \DP_{\hyperm}^{-2} \Psi
%	\bigl( \Id - \Pi_{\hyper} \bigr) \bigr\} .
%\label{E2IPikPTDGk}
%\end{EQA}
%The propagation condition for the prior \( \priorh_{\hyperm} \) reads as
%\begin{EQA}
%%	\sum_{\hyper > \hyperm} \riskt_{\hyperm}(\hyper) 
%	\E_{\hyperm} \bigl| \risktt_{\hyper} - \risktt_{\hyperm} \bigr|
%	& \leq &
%	\alp \riskt_{\hyperm} .
%%	\bigl( \bias_{\hyperm}^{2}(\hyperm) + \dimA_{\hyperm} \bigr) 
%\label{E1arttkksa}
%\end{EQA}
%for a fixed constant \( \alp \).
%
%\begin{theorem}
%\label{Tpriorpropag}
%The choice \( \priorh(\hyperm) =  \) ensures the propagation condition.
%\end{theorem}
%
%\begin{proof}
%Without loss of generality we assume that \( \Psi \Psi^{\T} = n \Id_{\dimp} \).
%Let us fix some \( \hyper \geq \hyperm \).
%Let \( \thetav \sim \ND(0,\GP_{\hyperm}^{-2}) \).
%We study the value of the corresponding squared relative bias 
%\( \bias_{\hyperm}^{2}(\thetav) - \bias_{\hyper}^{2}(\thetav) \).
%By \eqref{bikk2vakk2} for \( \fv = \Psi^{\T} \thetav \)
%\begin{EQA}
%	\bias_{\hyperm}^{2}(\thetav) - \bias_{\hyper}^{2}(\thetav)
%	&=&
%	\sigma^{-2} \bigl\langle \fv, (\Pi_{\hyper} - \Pi_{\hyperm}) \fv \bigr\rangle
%	=
%	\sigma^{-2} \bigl\langle \thetav, \Psi (\Pi_{\hyper} - \Pi_{\hyperm}) \Psi^{\T} \thetav \bigr\rangle .
%\label{s2b2kfsIPfPPT}
%\end{EQA} 
%The identity \( \Psi \Psi^{\T} = n \Id_{\dimp} \) imples
%\begin{EQA}
%	\Psi (\Pi_{\hyper} - \Pi_{\hyperm}) \Psi^{\T}
%	&=&
%	\Psi \Psi^{\T} \Bigl\{ 
%		\bigl( \Psi \Psi^{\T} + \sigma^{2} \GP_{\hyper}^{2} \bigr)^{-1} 
%		- \bigl( \Psi \Psi^{\T} + \sigma^{2} \GP_{\hyperm}^{2} \bigr)^{-1} 
%	\Bigr\} \Psi \Psi^{\T}
%	\\
%	&=&
%	n \Bigl\{ 
%		\bigl( \Id_{\dimp} + \sigma^{2} n^{-1} \GP_{\hyper}^{2} \bigr)^{-1} 
%		- \bigl( \Id_{\dimp} + \sigma^{2} n^{-1} \GP_{\hyperm}^{2} \bigr)^{-1} 
%	\Bigr\} .
%%	=
%%	\sigma^{2} \GP_{\hyper}^{2} \bigl( \Id_{\dimp} + \sigma^{2} n^{-1} \GP_{\hyper}^{2} \bigr)^{-1} .
%\label{s2nnIps2nm1Gk2}
%\end{EQA}
%If \( \thetav = \GP_{\hyperm}^{-1} \gammav \) with standard normal \( \gammav \), then
%\begin{EQA}
%	\bias_{\hyperm}^{2}(\thetav) - \bias_{\hyper}^{2}(\thetav) 
%	&=&
%	\bigl\langle \gammav, \BB_ {\hyper}(\hyperm) \gammav \bigr\rangle
%\label{bk2bgBhkmg}
%\end{EQA}
%and
%\begin{EQA}
%	\BB_{\hyper}(\hyperm)
%	& \eqdef &
%	n \sigma^{-2} \GP_{\hyperm}^{-1}  
%	\Bigl\{ \bigl( \Id_{\dimp} + \sigma^{2} n^{-1} \GP_{\hyper}^{2} \bigr)^{-1}
%		- \bigl( \Id_{\dimp} + \sigma^{2} n^{-1} \GP_{\hyperm}^{2} \bigr)^{-1} 
%	\Bigr\} 
%	\GP_{\hyperm}^{-1} .
%\label{BBhmGmm1Is2m1}
%\end{EQA}
%Gaussian concentration yields that 
%\( \bigl\langle \gammav, \BB_{\hyper}(\hyperm) \gammav \bigr\rangle \approx 
%\tr \BB_ {\hyper}(\hyperm) \). 
%One can easily see that the bias term \( \tr \BB_ {\hyper}(\hyperm) \) 
%decreases with \( \hyper \), while the variance term 
%\( \varA_{\hyper}^{2} - \varA_{\hyperm}^{2} \) increases. 
%Now we show that the sum \( \varA_{\hyper}^{2} + \tr \BB_{\hyper}(\hyperm) \) increases with 
%\( \hyper \geq \hyperm \).
%
%\begin{lemma}
%\label{Lhypermhi}
%It holds
%\begin{EQA}
%	\varA_{\hyper}^{2} + \tr \BB_{\hyper}(\hyperm)
%	&>& 
%	0 \, ,
%	\quad
%	\hyper > \hyperm .
%\label{vAkkmtBkkm}
%\end{EQA}
%\end{lemma}
%\begin{proof}
%Let both \( \GP_{\hyperm}^{2} \) and \( \GP_{\hyper}^{2} \) be diagonal and \( \Psi \Psi^{\T} = n \Id_{n} \). 
%Then
%\begin{EQA}
%	&& \nquad
%	\varA_{\hyper}^{2} + \tr \BB_{\hyper}(\hyperm)
%%	- \bigl( \varA_{\hyperm}^{2} + \tr \BB_ {\hyperm,\hyperm} \bigr)
%	\\
%	&=&
%	\sum_{j \geq 1} 
%	\biggl( 
%		- \log \frac{\sigma^{2} n^{-1} g_{j,\hyper}^{2}}{1 + \sigma^{2} n^{-1} g_{j,\hyper}^{2}} 
%		- \frac{1}{1 + \sigma^{2} n^{-1} g_{j,\hyper}^{2}}
%		+  \frac{g_{j,\hyper}^{2} \, g_{j,\hyperm}^{-2}}{1 + \sigma^{2} n^{-1} g_{j,\hyper}^{2}} 
%	\biggr)	
%\label{112m1gj1s2nm1} 
%\end{EQA}
%For each \( j \), define \( u = g_{j,\hyper}^{2} \, g_{j,\hyperm}^{-2} \leq 1 \), and \( c = \sigma^{2} n^{-1} g_{j,\hyperm}^{-2} \).
%Then
%\begin{EQA}
%	f(u)
%	& \eqdef &
%	- \log \frac{c u}{1 + cu} - \frac{1}{1 + c u} + \frac{u}{1 + cu}
%\label{fulcu1cuucu}
%\end{EQA}
%decreases in \( u \) whatever \( c > 0 \) is. 
%\end{proof}
%This result means that the systematic part \( \E_{\hyperm} \riskt_{\hyper} \) of the empirical quantity
%\( \risktt_{\hyper} \) is minimized for \( \hyper = \hyperm \).
%\end{proof}

\subsection{Partial ordering and anisotropic modeling}
Now we consider the case of a bivariate hyperparameter \( (\hyper, \HYPER) \in \MMs \times \TAU \).
We assume that the ordering condition \eqref{GPorderhh2} holds for each of parameters \( \hyper \), \( \HYPER \)
when the other is fixed arbitrarily.
 



 

